A Survey on Mixup Augmentations and Beyond

As Deep Neural Networks have achieved thrilling breakthroughs in the past decade, data augmentations have garnered increasing attention as regularization techniques when massive labeled data are unavailable. Among existing augmentations, Mixup and relevant data-mixing methods that convexly combine selected samples and the corresponding labels are widely adopted because they yield high performances by generating data-dependent virtual data while easily migrating to various domains. This survey presents a comprehensive review of foundational mixup methods and their applications. We first elaborate on the training pipeline with mixup augmentations as a unified framework containing modules. A reformulated framework could contain various mixup methods and give intuitive operational procedures. Then, we systematically investigate the applications of mixup augmentations on vision downstream tasks, various data modalities, and some analysis \& theorems of mixup. Meanwhile, we conclude the current status and limitations of mixup research and point out further work for effective and efficient mixup augmentations. This survey can provide researchers with the current state of the art in mixup methods and provide some insights and guidance roles in the mixup arena. An online project with this survey is available at https://github.com/Westlake-AI/Awesome-Mixup.

==> 0_Abstract.tex <==
\begin{abstract}
As Deep Neural Networks have achieved thrilling breakthroughs in the past decade, data augmentations have garnered increasing attention as regularization techniques when massive labeled data are unavailable. Among existing augmentations, Mixup and relevant data-mixing methods that convexly combine selected samples and the corresponding labels are widely adopted because they yield high performances by generating data-dependent virtual data while easily migrating to various domains.
This survey presents a comprehensive review of foundational mixup methods and their applications.
We first elaborate on the training pipeline with mixup augmentations as a unified framework containing modules. A reformulated framework could contain various mixup methods and give intuitive operational procedures.
Then, we systematically investigate the applications of mixup augmentations on vision downstream tasks, various data modalities, and some analysis \& theorems of mixup. Meanwhile, we conclude the current status and limitations of mixup research and point out further work for effective and efficient mixup augmentations. This survey can provide researchers with the current state of the art in mixup methods and provide some insights and guidance roles in the mixup area.
An online project with this survey is available at \url{https://github.com/Westlake-AI/Awesome-Mixup}.

\end{abstract}

\begin{CCSXML}
<ccs2012>
    <concept>
        <concept_id>10002978.10003022.10003023</concept_id>
        <concept_desc>Security and privacy~Software security engineering</concept_desc>
        <concept_significance>500</concept_significance>
        </concept>
   <concept>
       <concept_id>10011007.10011006.10011072</concept_id>
       <concept_desc>Software and its engineering~Software libraries and repositories</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
    <concept>
        <concept_id>10002978.10003006</concept_id>
        <concept_desc>Security and privacy~Systems security</concept_desc>
        <concept_significance>300</concept_significance>
        </concept>
    </ccs2012>
\end{CCSXML}


\ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

\keywords{Data Augmentation, Mixup, Classification, Self-supervised Learning, Computer Vision, Natural Language Processing}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

\maketitle

% developers are highly relying on DL libraries to develop DL-based software systems (software that contain DL components), and bugs in such libraries may be propagated to DL programs developed using those libraries.

==> 1_Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Deep Neural Networks (DNNs), such as Convolutional Neural Networks (CNNs) and Transformers, since their powerful feature representation ability that has been successfully applied to a variety of tasks, \emph{e.g.} Image Classification, Object Detection, and Natural Language Processing (NLP), \emph{etc.} To accomplish progressively more challenging tasks, DNNs employ a large number of learnable parameters, and that means that without numerous training data, models could easily get overfitting and fail to generalize. However, training data in some scenarios were unavailable and expensive to collect. Therefore, enabling DNNs to generalize beyond limited training data becomes one of the fundamental problems in deep learning. 

To address the data-hungry problem, researchers have proposed data augmentation (DA) techniques. Unlike ``model-centric" approaches, DA is a ``data-centric" method that alleviates overfitting by synthesizing virtual data. By creating varied versions of the same sample, DA introduces useful invariant features and provides inductive bias, thus enhancing regularization. Recent studies show that DA improves the generalization of deep learning models and is crucial for achieving state-of-the-art performance. 

In this survey, we focus on \textbf{Mixup}. 
MixUp~\cite{zhang2018mixup} generates augmented samples by interpolating two samples with their one-hot labels.
Most existing augmentation methods modify single samples without changing their labels. In contrast, Mixup generates augmented samples by combining features from two or more examples, resulting in multiple labels that better reflect real-world conditions. Mixup also shows strong transferability across different datasets and domains. Conversely, other combination methods often require significant time to identify effective augmentation strategies. Furthermore, generative methods can be difficult to apply to large datasets due to the need for additional generators and discriminators, which limits transferability and applicability. 
In contrast, Mixup does not rely on label-preserving operations but uses a learnable approach to generate virtual training data by combining multiple samples, producing a large of data without requiring domain knowledge.
Based on those advantages, mixup has been successfully applied to various tasks and training paradigms, including supervised learning (SL), self-supervised learning (SSL), semi-supervised learning (Semi-SL), texts, graphs, speech, and so on. Fig. \ref{fig: timeline} summarizes the timeline of mainstream methods within these training paradigms and data modalities.
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3]{Figs/pipeline.pdf}
    \caption{The mixup methods followed these steps: \textbf{(\romannumeral1).} Loading mini-batch raw samples from the training dataset; \textbf{(\romannumeral2).} For some downstream tasks, methods involve selecting and retaining reliable raw samples. Saliency-based or attention-based techniques use a pre-trained model to identify feature regions or tokens. The mixing ratio $\lambda$ is then defined by sampling from either a Beta or Uniform distribution. \textbf{(\romannumeral3).} After initialization, raw samples were mixed with other samples by sample mixup policies. \textbf{(\romannumeral4).} When the mixed samples $\hat{x}$, there were two choices: One was sampling, some methods updated the mixing ratio by mask $\mathcal{M}$ total pixels, some selected mixed samples for retaining more diversity or challenging samples, and some methods redefined the mixing ratio. Another was label mixup policies, we illustrate those policies in subsection 3.2 and further mining labels $\hat{y}$. \textbf{(\romannumeral5).} The final step involved channel mixup policies. Mixed samples $\hat{x}$ were encoded by the network and mapped into a high-dimensional latent space. Some methods interpolated these features or selected feature maps to generate high-dimensional features $\hat{z}$. These features were then further encoded into feature vectors for different tasks, and optimized using various loss functions.}
    \vspace{-20pt}
    \label{fig: pipeline}
\end{figure}

Overall, compared to three published surveys ~\cite{cao2022mixup-survey1}, ~\cite{lewy2023mixup-survey2} and ~\cite{naveed2024mixup-survey3} on Mixup, our contributions include:
\begin{itemize}
    \item We provide a timely literature review and a comprehensive framework to conceptualize two different improvement strategies (Sample and Label) for the mixup method, using SL as an example. These two strategies could correspond to different training paradigms and data modalities.

    \item We carefully review and discuss the details of the techniques of various categories of mixup methods, such as Static Linear, Saliency-based, Attention-based, \emph{etc.}, to give researchers a better overview of the method involved, leading to further understanding and insights.

    \item We report a systematic survey of the application of mixup methods to downstream tasks, propose technical challenges and further demonstrate their broad applicability to other modalities and domains beyond vision tasks, \emph{e.g.}, audio, speech, graphics, biology, \emph{etc}.

    \item We further summarize the mixup method as a trainable paradigm, compared to other surveys that utilize it as the DA tool and methods. We appeal to researchers to contribute a unified framework for mixup to address a variety of tasks, rather than discrete task-specific modifications.
    
\end{itemize}


==> 2_Preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

\subsection{Notions}
\begin{wraptable}{r}{0.5\textwidth}
    \centering
    \vspace{-1.3em}
    \input{Tabs/notions}
\end{wraptable}
Table \ref{Notion} and Table \ref{Abbreviations} list the notations and abbreviations used in this survey. We define a total sample set as $\mathbb{X} \in \mathbb{R}^{C \times W \times H}$, and corresponding label set as $\mathbb{Y} \in \mathbb{R}^{k}$. In Computer Vision (CV) tasks, $x \in \mathbb{X}^{C \times W \times H}$, in NLP tasks, $x \in \mathbb{X}^{C \times L}$, where $L$ denotes the original sentence, and in Graph Neural Network (GNN) tasks, $v$ noticed as a node and $\mathcal{V}$ represent the distribution of its neighborhood. In mixup methods, $\hat{x}$ and $\hat{y}$ denote mixed samples and labels, respectively. $\lambda$ denotes the mixing ratio that samples from Beta or Uniform distribution. In addition, we use $\mathcal{M} \in \{0, 1\}$ to represent the mask obtained from some Ad-Hoc or Adaptive methods. Training models denotes $f_\theta(\cdot)$, where $\theta$ is learnable parameters. $f^\prime(\cdot)$ denotes pre-trained or teacher models, and $f^\star_\theta(\cdot)$ denotes optimized model fixed from $f_\theta(\cdot)$. In SSL or Semi-SL, $\tau$ denotes the temperature used for the Sharpen function or scaling of the pseudo-labels.
% \input{Tabs/notions}

\subsection{Mixup Framework Modules}
In this subsection, we will detail each module's functions in the mixup method pipeline, as shown in Fig. \ref{fig: pipeline}.

\textbf{(\romannumeral1). Initialization.} Before mixup, some methods select raw samples within the mini-batch to filter those suitable for mixing, \emph{e.g.} Co-Mix~\cite{kim2020co} selected suitable samples in the mini-batch to maximize the diversity of the mixed samples obtained. Additionally, some saliency-based methods used pre-trained models to locate and obtain feature maps. Finally, each method obtained the mixup ratio $\lambda$ from the Beta distribution. 

\textbf{(\romannumeral2). Sample Mixup Policies.} In Supervised Learning, we divide the policies into 9 classes and we detail these classes in Fig. \ref{mixup4cv}. \textbf{Static Linear} methods used $\lambda$ mixed two or more samples based on interpolation linear. \textbf{Fearture-based} methods used raw samples feature maps obtained by $f_\theta(\cdot)$, and mixed them in interpolation linear. \textbf{Cutting-based} methods are used in various ways such as cutting, resizing, or stacking to mix samples, with the mixing ratio $\lambda$ from the mask area. \textbf{K Sample mixup} methods used more than 2 samples mixing. \textbf{Random Policies} methods combined lots of different augmentation methods and some hand-crafted mixup methods, the policy is chosen by each method's weight factor. \textbf{Style-based} mixed samples from their style and content by an additional style extractor. \textbf{Saliency-based} methods used sample feature maps to locate their saliency information and obtained max feature mixed samples. \textbf{Attention-based} methods, similar to saliency-based methods, utilized attention scores rather than saliency maps. \textbf{Generating Samples} used some generative models such as GAN-based models~\cite{goodfellow2020gans} and Diffusion-based models~\cite{brooks2023instructpix2pix} to generating mixed samples.
    
\textbf{(\romannumeral3). Label Mixup Policies.} We divide into 8 classes in SL and also display them in Fig. \ref{mixup4cv} detailed. \textbf{Optimizing Calibration} methods used the ECE metric to rank the mixed samples and selected them for improving classification performance and model calibration. \textbf{Area-based} methods used mask region redefine mixing ratio $\lambda$. \textbf{Loss Object} methods redefined a new mixup classification loss or proposed a new loss as a regularization method. \textbf{Random Policies} methods combined the other augmentation methods with mixup methods or proposed new training strategies for the mixup. \textbf{Optimizing Mixing Ratio} methods used learnable parameter as $\lambda$, obtained reliable mixing ratio by different mixed samples. \textbf{Generating Label} methods generated mixed labels by mixed samples rather than using one-hot labels. \textbf{Attention Score} methods used attention maps from raw samples to determine the mixing ratio or utilized attention maps from mixed samples to compute the ratio based on scores from each sample. \textbf{Saliency Token} methods used each raw sample's saliency maps and divided them into tokens, computed mixing ratio by tokens used.
    
\textbf{(\romannumeral4). Sampling.} Some methods focus solely on sample policies to enhance model performance and capability. These methods used various strategies to fix the ratio $\lambda$ or the labels. Some computed the ratio $\lambda$ based on all pixels in the mask, while others set a weight factor for mixed samples.
    
\textbf{(\romannumeral5). Channel Mixup Policies.} Different from samples or labels, channels with lots of high-level features. Manifold Mixup~\cite{verma2019manifold} obtained mixed samples by interpolation linear, and Catch up-Mix~\cite{kang2024catchupmix} obtained mixed samples by selecting some feature maps for further improving filter capacity.


==> 3_Mixup_Methods4CV_tasks.tex <==
\section{Mixup Methods for CV tasks}
\label{sec:mixup4cv}
This section focuses on mixup methods used for CV tasks. We reviewed widely of these methods and divided them into four categories: \textbf{(1)} Supervised Learning, \textbf{(2)} Self-Supervised Learning, \textbf{(3)} Semi-Supervised Learning, and \textbf{(4)} some mainstream downstream tasks in the CV: Regression, Long-tail, Segmentation, and Object Detection. 
Fig. \ref{fig: sample_mixup_policies} and Fig. \ref{fig: label_mixup_policies} summarise some mixup methods in SL tasks.

\subsection{Sample Mixup Policies in SL}
\label{sec:3.1}
\subsubsection{\textbf{Static Linear}}
\label{sec:3.1.1}
Static Linear methods use ratios to interpolate globally linearly to get mixed samples. Where MixUp~\cite{zhang2018mixup} is the seminal work of mixup-based methods, as shown in Eq. \ref{eq:1}, the
efficient and simple methods can bring immediate performance to the model. At the same time, BC~\cite{cvpr2018bc} also proposed a similar process to MixUp. Unlike MixUp, which obtained the mixing ratio $\lambda$ from the Beta distribution, BC chose to receive $\lambda$ from the Uniform distribution.
\begin{equation}
    \begin{aligned}
    \label{eq:1}
        \hat{x} = \lambda * x_i + (1-\lambda) * x_j, \ \hat{y} = \lambda * y_i + (1-\lambda) * y_j.
    \end{aligned}
\end{equation}
AdaMixup~\cite{guo2018adamix} and Local Mixup~\cite{baena2022localmixup} further considered the problem of \emph{``Manifold Intrusion"}. AdaMixup used a learnable ratio to get reliable mixed samples and Local Mixup mining mixed sample pairs ($x_i, x_j$) by weighting the training losses of the mixed samples with $w$. 
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figs/samples_mixup_policies.pdf}
    \caption{Illustration of sample mixup policies in SL, we divided them into two branches: \textbf{Ad-Hoc} and \textbf{Adaptive}, and divided them into nine types detailed.}
    \vspace{-10pt}
    \label{fig: sample_mixup_policies}
\end{figure*}
\subsubsection{\textbf{Feature-based}}
\label{sec:3.1.2}
Feature-based methods transfer mixup methods from pixel-level to latent-level. Manifold Mixup~\cite{verma2019manifold} used the ratio $\lambda$ linearly mixing the sample features from the input samples encoded by models:
\begin{equation}
    \label{eq:3}
    \begin{aligned}
        \hat{z} & = \lambda * f_\theta(x_i) + (1-\lambda) * f_\theta(x_j),
    \end{aligned}
\end{equation}
where the $f_\theta(\cdot)$ denotes encoder, and the $\hat{z}$ denoted the mixed features. However, PatchUp~\cite{faramarzi2020patchup} chose to use the generated mask to mask features in Hard PatchUp or Soft PatchUp. The Hard PatchUp indicates that the mask is binary, and the Soft PatchUp way indicates that the mask is $\lambda$-valued similarly:
\begin{equation}
    \label{eq:4}
    \begin{aligned}
        \left\{\begin{matrix} 
          \mathcal{M}_h = 1,  & \text{Hard\ PatchUp}, \\  
          \mathcal{M}_s = \lambda, & \text{Soft\ PatchUp},
        \end{matrix}\right.
    \end{aligned}
\end{equation}
\begin{equation}
    \label{eq:5}
    \begin{aligned}
        \hat{z} & = \mathcal{M}_{h/s} \odot f_\theta(x_i) + (1 - \mathcal{M}_{h/s}) \odot f_\theta(x_j),
    \end{aligned}
\end{equation}
where the $\mathcal{M}_{h/s}$ denotes the mask which obtained from Eq. \ref{eq:4}, and the $\odot$ is element-wise multiplication. MoEx~\cite{li2021moex} operated on the training image in feature space, exchanging the moments of the learned features between images and interpolating the target labels. The mixing ratio $\lambda$ are used to combine the Mixup Cross-Entropy (MCE) loss function by Eq. \ref{eq:6}:
\begin{equation}
    \label{eq:6}
    \begin{aligned}
        \mathcal{L}_{MCE} & = \lambda * \mathcal{L}(z^{(j)}_i, y_i) + (1-\lambda) * \mathcal{L}(z^{(j)}_i, y_j),
    \end{aligned}
\end{equation}
where the $z^{(j)}_i$ denotes the feature representation of $x_i$, which has been injected with the moments of $x_j$. In another way, Catch-up Mix~\cite{kang2024catchupmix} proposed a filtering module mixing the features learned by poor filters to obtain mixed features, which further improves their capabilities.

\subsubsection{\textbf{Cutting-based}}
\label{sec:3.1.3}
Cutting-based methods used some masks to mix samples. Unlike Cutout drops a patch in samples, CutMix~\cite{yun2019cutmix} randomness generated rectangular binary masks $\mathcal{M}$ and mix samples according to Eq. \ref{eq:7}:
\begin{equation}
    \label{eq:7}
    \begin{aligned}
        \hat{x} & = \mathcal{M} \odot x_i + (1 - \mathcal{M}) \odot x_j,
    \end{aligned}
\end{equation}
where the $\mathcal{M} \in \frac{r_w r_h}{WH}$, and $r_w = W \sqrt{1-\lambda}$, $r_h = H \sqrt{1-\lambda}$. GridMix~\cite{Baek2021gridmix} and MixedExamples~\cite{summers2019mixedexamples} used grid masks similar to GridMask, rather than a single patch to obtain mixed samples. SmoothMix~\cite{lee2020smoothmix} proposed a smoothing mask for mixing samples with a smooth boundary. Similarly,  StarMix~\cite{jin2024starlknet} employed a smooth mask for mixing samples for the vein identification task. 
SuperGridMix~\cite{hammoudi2022superpixelgridcut} used Superpixel segmentation methods to get the mask. MSDA~\cite{park2022msda} used MixUp and CutMix to obtain mixed samples. ResizeMix~\cite{qin2020resizemix} asserts that, regardless of the cutting or blending method used, there is a risk of losing source sample features due to randomness. However, the resize method is designed to retain the complete information of the source sample while maximizing the feature information of the mixed samples, as described by Eq. \ref{eq:8}:
\begin{equation}
    \label{eq:8}
    \begin{aligned}
        \hat{x} = \mathcal{P}(T(x_i, \lambda_\tau), x_j),\
        \hat{y} = \lambda * y_i + (1-\lambda) * y_j,
    \end{aligned}
\end{equation}
where $T(\cdot)$ denotes the resizing function and the scale rate $\lambda_\tau$ is sampled from the uniform distribution $\lambda_\tau \sim U(\alpha, \beta)$.
$\mathcal{P}(\cdot)$ denotes paste the score sample $x_i$ to the target sample $x_j$. The $\lambda$ is defined by the size ratio of the patch and target sample.
Unlike pixel-level mixing, FMix ~\cite{harris2020fmix} argues that effective features are often continuous in an image. Therefore, samples are transformed into Fourier space using the Fourier transform to sample high and low-frequency information, generating binary masks. Pani MixUp ~\cite{sun2024panimixup} interpolated mixing by GNNs to build relationships between sample patches. Moreover, instead of using mask-based ways, some works, \emph{e.g.} StackMix~\cite{chen2022stackmix}, RICAP~\cite{takahashi2019ricap}, YOCO~\cite{han2022yoco} stacking samples directly. Some cutting-based mixup methods are shown in Fig. \ref{fig: cut_resize_satck}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figs/sl_methods.pdf}
    \caption{Illustration of simplifying the flow of sample mixup policies in supervised learning (SL). Note that $x_i$ and $x_j$ denote different samples, $z$ denotes feature maps, $\hat{x}$ denotes mixed sample, $\lambda$ was the mixing ratio, and $\mathcal{M}$ denotes mask. (a) \textbf{Static Linear} interpolates samples directly; (b) \textbf{Feature-based} interpolates sample's feature maps; (c) \textbf{Cutting-based} uses cut or resize way mixing samples; (d) \textbf{K Samples Mixup} mixing more than two samples; (e) \textbf{Random Policies} randomly choose mixup policy; (f) \textbf{Style-based} uses a style-transfer encoder to extract content and style and decode the mixed samples; (g) \textbf{Saliency-based} and (h) \textbf{Attention-based} apply a per-train CNN or ViT, mixing samples according to the saliency map or attention score; (i) \textbf{Generating Sample} uses Generative Models to obtain mixed samples.}
    \vspace{-5pt}
    \label{fig: sample_method}
\end{figure}
\subsubsection{\textbf{K Samples Mixup}}
\label{sec:3.1.4}
Many mixup methods focus on mixing two samples, with little analysis of how mixing more than two samples impacts model performance. $k$-mixup~\cite{greenewald2021kmixup} created additional mixed samples by interpolating under the Wasserstein metric and perturbing $k$-batches in terms of the other K samples. DCutMix~\cite{jeong2021dcutmix} obtained mixed samples by applying CutMix multiple times. Experimental analyses of multi-mixed samples showed that multi-sample mixing of Landspace guided the model towards the widest (flattest) and deepest local minima. MixMo~\cite{rame2021mixmo} proposed a multi-input, multi-output (MIMO) model that fuses MixUp with an integrated MIMO model to find the best mixing network to handle multiple sub-networks.
Some works \emph{g.g.} RICAP, Cut-thumbnail~\cite{xie2021Cut-thumbnail}, Mosaic~\cite{redmon2016yolo} obtained mixed samples to improve model's performance by stacking or cutting multi-samples.

\subsubsection{\textbf{Random Policies}}
\label{sec:3.1.5}
RandomMix~\cite{liu2024randomix} combined MixUp, CutMix, ResizeMix, and FMix into a policy set, randomly choosing one of them and their weight to get mixed samples. Furthermore, AugRMixAT~\cite{liu2022augrmixat}, adds additional augmentation methods and adversarial attack aim to get a more robust model.

\subsubsection{\textbf{Style-based}}
\label{sec:3.1.6}
\textbf{Static ways.} AugMix~\cite{hendrycks2019augmix} aimed to improve model robustness and uncertainty estimation by using randomness and multiple augmentation methods to mix samples. The model is trained using the Jensen-Shannon divergence loss for consistency, as defined in Eq. \ref{eq:2}:
\begin{equation}
    \label{eq:2}
    \begin{aligned}
        \hat{x} & = \lambda*(\textrm{w}_i*\mathcal{A}(x_i) + \textrm{w}_j*\mathcal{A}(x_j)) + (1-\lambda)*x_z,
    \end{aligned}
\end{equation}
where $\textrm{w}_i$, and $\textrm{w}_j$ are randomly generated weights from the Dirichlet distribution. PixMix~\cite{hendrycks2022pixmix} and IPMix~\cite{huang2024ipmix} further improved AugMix by mixing additional fractals datasets with the samples, mixing with a $\mathcal{A}(x)$, and repeating this several times to get the final mixed samples. This is used to tackle some Out-of-Distribution (OOD) scenarios and improve the robustness of the model. DJMix~\cite{hataya2020djmix} also extended AugMix by using a mixture of the input image and the discretized image.

\textbf{Dynamic ways.} StyleMix~\cite{cvpr2021stylemix} proposed the concept of differentiating and mixing the content and style features of input image pairs to create more abundant and robust samples. 
Specifically, StyleMix employed the adaptive instance normalization layer (AdaIN)~\cite{Huang2017ArbitraryST} to exchange styles for images $x_i$ and $x_j$ (Eq. \ref{eq:9}). To obtain a new mixed image $\hat{x}$, StyleMix linearly interpolates feature maps with a content ratio $\lambda_c$ and a style ratio $\lambda_s$ by Eq. \ref{eq:10}. 
\begin{equation}
    \label{eq:9}
    \begin{aligned}
       \hat{z}_{i,j}  = \sigma(z_j)(\frac{z_i-\mu(z_i)}{\sigma(z_i)})+\mu(z_j),
    \end{aligned}
\end{equation}
\begin{equation}
    \label{eq:10}
    \begin{aligned}
       \hat{x}  & = \text{De}( \nu(z_i)+( 1 - \lambda_c - \lambda_s + t))z_j +(\lambda_c - \nu ) \hat{z}_{i,j} + (\lambda_s - \nu )\hat{z}_{j,i},
    \end{aligned}
\end{equation}
where $\hat{z}_{i,j}$ has the content component of $x_i$ and the style of $x_j$, $\text{De}(\cdot)$ is the pre-trained style decoder and $\nu \in [\max(0,\lambda_c + \lambda_s - 1),\min(\lambda_c, \lambda_s)]$ is a variable. MixStyle~\cite{zhou2021mixstyle} was inspired by AdaIN, which effectively combines style transfer and mixup across source domains. 
Unlike StyleMix ~\cite{cvpr2021stylemix}, MixStyle does not include a decoder for image generation. Instead, it perturbs the style information of source domain training instances to implicitly synthesize novel domains.

AlignMixup~\cite{2021alignmix} obtained the mixed feature maps by using assignment matrix $M_R$, which Sinkhorn-Knopp obtains ~\cite{knight2008sinkhorn} on similarity matrix $e^{-M/\tau}$. $z_j$ is aligned to $z_i$ according to $M_R$, giving rise to $z^\prime_j$=$M_R(z_j)$, then interpolate between $z_i$, $z^\prime_j$. MultiMix~\cite{venkataramanan2022multimix} obtained augmented feature maps by additional attention and $\lambda$ element-wise multiplication of the matrix $M_a$, and obtained mixed feature maps by Eq. \ref{eq:13}:
\begin{equation}
    \label{eq:13}
    \begin{aligned}
       \hat{z} & = \textrm{norm}(M_a(\textrm{A}_i, \lambda)) \odot z_i  + \textrm{norm}(M_a(\textrm{A}_j, 1-\lambda) \odot z_j,
    \end{aligned}
\end{equation}
where $\textrm{norm}(\cdot)$ denotes normalization, and $\textrm{A}$ is obtained from $z$ after GAP (Global Average Pooling) or $z$ after CAM (Class Activation Maps)~\cite{selvaraju2017grad} calculation.

\subsubsection{\textbf{Saliency-based}}
\label{sec:3.1.7}
Saliency-based methods to maximize features in the mixed samples use additional feature extractors or backward gradient obtained saliency maps~\cite{simonyan2014saliency} to locate feature locations to guide mask $\mathcal{M}$ generation. 

\textbf{Additional Feature Extractor.} SaliencyMix~\cite{uddin2020saliencymix} used a feature extractor to select the peak salient region from the saliency map in the source image and mix the source patch with the target image. Attentive-CutMix~\cite{icassp2020attentive} used a pre-trained classification model $f^\prime _\theta(\cdot)$ as a teacher model aims to generate a mask of source sample feature patches, first obtain a heatmap of the source image, then select the top-$N$ patches from this map as attentive region patches to cut from the source image. Similarly, FocusMix~\cite{kim2020focusmix} used CAM to generate masks for mixed samples. AttributeMix~\cite{li2020attributemix} build a $K$-Dictionary to get a different feature on each sample and mix for the fine-grained classification task. GraSalMix~\cite{hong2023gradsalmix} was found to locate feature regions in the samples more accurately based on network gradient than CAM and used cutting-based mixing for the $z$ obtained for each network stage. RecursiveMix~\cite{yang2022recursivemix} advised to keep historical samples for mixing. Use RoI and ResizeMix to mix samples iteration by iteration.

PuzzleMix~\cite{kim2020puzzle} first feeds the samples into the model to obtain the gradient, then backpropagates this gradient to generate a saliency map. Based on this map, the samples are divided into multiple patches, and masks are generated with a ratio $\lambda$ corresponding to the number of patches. To prevent the problem of feature loss due to two sample features at the same location, Kim. \emph{et al.} 
proposed Co-Mix~\cite{kim2020co}. Instead of being limited to mixing between pairs of samples ($x_i, x_j$), the mixup process is guided by finding multiple samples in a mini-batch for mixing and turning the search for the optimal mixup method into an optimization problem through multiple mixed samples. To improve the diversity of mixed samples, a regularization loss is introduced to penalize the generation of overly similar images. GuidedMixup~\cite{kang2023guidedmixup} proposed a greedy pairing algorithm to find the best sets with large distances between salient regions within the mini-batch images. The token-level approach is transferred to the pixel level to maximize saliency.
SuperMix~\cite{wu2023supermix} used a pre-trained model as a teacher to sample and generate a set of masks from a Dirichlet distribution, optimizing these masks with the Newton method. LGCOAMix~\cite{dornaika2023lgcoamix} used the superpixel method to obtain mixed samples, recalculated $\lambda$ using feature maps, and employed pooling and a self-attention module to derive local classification and superpixel contrastive losses.

\textbf{End-to-End way.} Using saliency or gradient information often incurs additional time overhead. AutoMix ~\cite{liu2022automix} used an end-to-end method to achieve optimal mixed samples in terms of both time efficiency and network performance. AutoMix proposed a lightweight generator, Mixblock, to automatically generate masks according to Eq. \ref{eq:14}:
\begin{equation}
\label{eq:14}
    \begin{aligned}
        \hat{x} = \mathcal{M}_\theta(z^l_{i,\lambda},z^l_{j,1-\lambda})\odot x_i + (1 - \mathcal{M}_\theta(z^l_{i,\lambda},z^l_{j,1-\lambda}))\odot x_j,
    \end{aligned}
\end{equation}
where $z^l_{i, \lambda}$ denotes $\lambda$ embedded feature maps at $l$-th layer. $\mathcal{M}_\theta$ denotes the Mixblock module with learnable parameters $\theta$. SAMix~\cite{li2021samix} further improves Mixblock and extends AutoMix in supervised learning tasks to self-supervised tasks. TransformMix~\cite{cheung2024transformmix} used a teacher model obtained samples CAMs and mixing by a new mixing module. AdAutoMix~\cite{qin2023adautomix} used adversarial training to obtain more challenging samples and improve the classification model's ability. It introduced a new Mixblock that enables mixing $N$ samples instead of two.

\subsubsection{\textbf{Attention-based}}
\label{sec:3.1.8}
Inspired by Vision Transformer (ViT)~\cite{iclr2021vit}, attention score maps also can be metrics such as CAM or gradient. TransMix~\cite{chen2022transmix} re-calculated the $\lambda$ by the area attention score of each sample. TokenMixup~\cite{choi2022tokenmixup} and TokenMix~\cite{liu2022tokenmix} selected the top-$N$ high-scoring tokens from the sample's attention map to use as masks, and $N= \lambda \mathbb{N}$.
ScoreMix~\cite{stegmuller2023scorenet} and SMMix~\cite{chen2023smmix} used the maximum and minimum attention regions of the sample attention map to mix samples by cutting the target sample maximum region and paste into the source sample minimum region to retain more feature information.

\subsubsection{\textbf{Generating Samples}}
\label{sec:3.1.9}
AAE~\cite{liu2018aae} obtained mixed samples by using the GANs model, first generating mixed feature maps similar to Manifold Mixup, and then using a Decoder to generate mixed samples, $\hat{z} = \lambda * \text{En}(x_i) + (1-\lambda) * \text{En}(x_j)$, $\hat{x} = \text{De}(\hat{z})$. And like GANs, AAE used a Discriminator to get adversarial loss, and total loss according to Eq. \ref{eq:15}:
\begin{equation}
    \label{eq:15}
    \begin{aligned}
    \mathcal{L}_{total} & = \mathcal{L}_{rec}(\vert\vert x - \hat{x} \vert\vert_{2}) + \mathcal{L}_{adv} (\log \text{Dis}(\hat{z}) + (1-(\log \text{Dis}(\hat{z})))
    ),
    \end{aligned}
\end{equation}
where $\mathcal{L}_{rec}$ denotes the reconstruction loss, and $\mathcal{L}_{adv}$ denotes the adversarial loss.
Similarly, AMR~\cite{beckham2019amr}, ACAI~\cite{berthelot2018acai}, AutoMixup~\cite{zhu2020automixup}, and VarMixup~\cite{mangla2020varmixup} all used generative models such as AE, VAE~\cite{kingma2013vae}, and GAN to interpolate feature maps in the latent space, then pass through a decoder to get the generated mixed samples. Inspired by the Text-to-Image model, 
DiffuseMix~\cite{islam2024diffusemix} used the Stable Diffusion-based multilingual model Instructpix2pix~\cite{brooks2023instructpix2pix}. This model obtained initial augmented samples using defined prompts and then generated the final mixed samples using YOCO and PixMix. DiffMix~\cite{wang2024diffmix} proposes an inter-class DA method that enriches the dataset by performing image transformations between classes, aims to address the correct foreground objects but not diverse backgrounds in generative models.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figs/label_mixup_policies.pdf}
    \caption{Illustration of label mixup policies in SL, we divided them into 8 types detailed.}
    \vspace{-10pt}
    \label{fig: label_mixup_policies}
\end{figure*}
\subsection{Label Mixup Policies in SL}
\subsubsection{\textbf{Optimizing Calibration}}
\label{sec:3.2.1}
Calibration measures how well a model's confidence aligns with its accuracy. A model should neither be overconfident nor underconfident, as this can lead to incorrect decisions. The Expected Calibration Error (ECE) is a key metric for evaluating model calibration. Manifold Mixup found that MixUp significantly improves network confidence but also noted that overconfidence is undesirable.
CAMixup~\cite{wen2020camix} found that a straightforward application of MixUp with Cross-Entropy (CE) loss increases the model's ECE, contrary to common expectations. Wen \emph{et al.} used Label Smoothing to verify that this is a labeling issue. CAMixup adjusted the mixing ratio based on the difference between the average accuracy and confidence of class classifications $\lambda$.

Normally, the model is expected to be more confident in predicting simpler classes. For harder classes, the model is encouraged to be less confident.
RankMixup~\cite{noh2023rankmixup} proposed a Mixup-based Ranking Loss (MRL):
\begin{equation}
    \label{eq:16}
    \begin{aligned}
        \mathcal{L}_{MRL} = \max(0, \max \hat{p}_i^k - \max p_i^k + m),
    \end{aligned}
\end{equation}
where $\hat{p}_i^k$ is a predicted probability of the class $k$ for the mixed sample $\hat{x}_i$, margin $m$ determines acceptable discrepancies between the confidences of raw and augmented samples. It encourages the confidence level of mixed samples to be lower than that of raw samples to maintain the ranking relationship. The goal is for higher confidence values to favor larger mixed samples, ensuring that confidence values are proportional to the mixing ratio.
SmoothMixup~\cite{jeong2021smoothmixup} using the inherent robustness of smoothing classifiers to identify semantically non-categorical samples and to improve the performance of classifiers.

\subsubsection{\textbf{Area-based}}
\label{sec:3.2.2}
RICAP~\cite{takahashi2019ricap} used the area of each sample in the mixed sample to calculate the $\lambda$. Some hand-crafted methods like CutMix, ResizeMix, and StackMix, \emph{ect.} use the mask area to calculate the $\lambda$. RecursiveMix similarly uses the history region to calculate the $\lambda_i = \sum \mathcal{M}_i$ for the mixed labels.

\subsubsection{\textbf{Loss Object}}
\label{sec:3.2.3}
Before describing the relevant methods, it is important to understand the loss function in the mixup task:
\begin{equation}
    \label{eq:17}
    \begin{aligned}
        \mathcal{L}_{MCE} = \lambda \mathcal{L}_{CE}(f_\theta(\hat{x}), y_i) + (1-\lambda) \mathcal{L}_{CE}(f_\theta(\hat{x}), y_j). 
    \end{aligned}
\end{equation}

In mixup tasks, the Softmax function can weaken the information of one class. When one of the $\lambda$ is too high, it can result in high entropy and low confidence, significantly affecting the prediction of a single class.
Liu \emph{et. al} proposed DecoupledMix~\cite{liu2022decoupledmix}, an effective loss function for mixup methods that includes adaptive ``hard-sample'' mining. Specifically, they separate the two classes in mixup, remove the probability $p$ from the denominator during the final softmax prediction, and use a two-hot encoding for regularization, as shown in Eq. \ref{eq:18}:
\begin{equation}
    \label{eq:18}
    \begin{aligned}
    \phi\left(z_{(i, j)}\right)^{a, b} & = \frac{\exp (z_{(i, j)}^{a} )}{\bcancel{\exp (z_{(i, j)}^{b} )}+\sum_{c \neq b} \exp (z_{(i, j)}^{c} )}, \quad
    \mathcal{L}_{DM} = -y_{[i, j]}^{T} \log (\phi (z_{(i, j)} ) ) y_{[i, j]},
    \end{aligned}
\end{equation}
where $\phi(\cdot)$ is the proposed decoupled Softmax, $(a,b)$ denotes the classes of the mixed samples, and $y_{[i, j]}$ is two-hot label encoding.
MixupE ~\cite{zou2023mixupe} analyzed mixup methods and found implicit regularization, proposed 2nd-order replacement, and introduced an improved method for enhancing effect.

\subsubsection{\textbf{Random Policies}}
\label{sec:3.2.4}
To address the slow convergence of mixup and the difficulty in selecting the mixing parameter 
$\alpha$, Yu \emph{et al.} proposed the mixup without hesitation (mWh)~\cite{yu2021mwh} method. This approach accelerates mixup by periodically disabling it. mWh analyzed and demonstrated through experiments that mixup is effective in early epochs but may become detrimental later. Thus, the mixup is gradually replaced by basic DA to shift from exploration to exploitation.

\subsubsection{\textbf{Optimizing Mixing Ratio}}
\label{sec:3.2.5}
AdaMixup~\cite{guo2018adamix} argues that simple interpolation to obtain mixed samples can lead to \emph{``Manifold Intrusion"}, where the mixed samples are too similar to raw samples of other classes.
Experiments found that the model performance is most affected at $\lambda$=0.5. Thus, AdaMixup proposed a method to learn $\lambda$. Two neural networks are introduced to generate the mixing ratio $\lambda$ and to judge whether the mixed samples cause \emph{``Manifold Intrusion"}. MetaMixup~\cite{mai2021metamixup} used Meta-Learning to optimize the mixup. The aim is a bi-fold optimization: the model $f_\theta(\cdot)$ and the $\lambda$. 

LUMix ~\cite{sun2022lumix} addressed label noise in the mixup process differently from previous methods. It proposed two approaches: detecting significant targets from the prediction and adding random samples from a uniform distribution to the label distribution to simulate label uncertainty. The final ratio is denoted as $\lambda$ = $\lambda_{0}*(1 - \nu_s- \nu_r) + \lambda_{s}*\nu_s + \lambda_{r}*\nu_r$, where $\lambda_{0}$ is set manually, $\lambda_{s}$ is calculated from the predictive distribution according to Eq. \ref{eq:19}, and $\lambda_{r}$ is sampled from $\text{Beta}(\alpha, \alpha)$.
\begin{equation}
    \label{eq:19}
    \begin{aligned}
    \hat{p}_{i} & =\frac{e^{p_i}}{\sum_{c=1}^{k} e^{p_c}}, \ \lambda_{s} =\frac{\hat{p}_i}{\hat{p}_i + \hat{p}_j},
    \end{aligned}
\end{equation}
and SUMix~\cite{qin2024sumix} is similar to LUMix in that it is assumed that it can be modeled in prediction to get a proper $\lambda$. In addition, SUMix applied the idea of metric learning to regularize the loss function by capturing the uncertainty in the samples.

\subsubsection{\textbf{Generating Label}}
\label{sec:3.2.6}
Simply interpolating the samples linearly may lead to the problem of \emph{``Manifold Intrusion"}. GenLabel~\cite{sohn2022genlabel} proposed to relabel the mixed samples. Firstly, learning the class-conditional data distribution using generative models for each class $c$, denoted as $p_c(x)$. Then, based on the likelihood $p_c(\hat{x})$ of the mixed samples extracted from each class $c$, the mixed samples are re-generated with the label $y^{gen}$ after obtaining the similarity according to Eq. \ref{eq:20}:
\begin{equation}
    \label{eq:20}
    \begin{aligned}
    y^{gen} & = \sum_{c=1}^{k} \frac{p_{c}(\hat{x})}{\sum_{c^{\prime}=1}^{k} p_{c^{\prime}}(\hat{x}) }e_c,
    \end{aligned}
\end{equation}
where $p_c(\hat{x})$ denotes density estimated for input feature $x \in \mathbb{X}$, conditioned on class $c \in [k]$, $k$ is the total classes.

\subsubsection{\textbf{Attention Score}}
\label{sec:3.2.7}
When using ViTs for classification, a class token is typically added, and the final prediction is based on this token after the model processes the input. However, this approach limits the utilized features to just the final class token, despite generating multiple feature tokens from the raw image, thus reducing the effectiveness of supervision. Token Labeling ~\cite{jiang2021tokenlabeling} labels all tokens in ViTs for classification tasks. Compared to the original loss function, Token Labeling adds the classification loss for all tokens:
\begin{equation}
    \label{eq:21}
    \begin{aligned}
    \mathcal{L}_{total} & = \mathcal{L}_{CE}(p^{cls}, y) + \textrm{w} * \frac{1}{\mathbb{N}} \sum^{\mathbb{N}}_{i=1}\mathcal{L}_{CE}(\textrm{token}_i, y_i),
    \end{aligned}
\end{equation}
where the $p^{cls}$ denotes the predication of the class token, and $\textrm{token}_i$ denotes the predication of the $i$-index token. TokenMix~\cite{liu2022tokenmix} and TokenMixup~\cite{choi2022tokenmixup} used the raw samples attention score for calculating the $\lambda$ of classes.
Mixpro~\cite{zhao2023mixpro} argued that attention scores obtained in the early stages are inaccurate and provide incorrect information. Therefore, it proposed a progressive factor that combines region and attention scores to calculate $lambda$.
Differ from MixPro, TL-Align~\cite{xiao2023tl-align} used the mixed samples into the ViTs when each layer is through $\bm{M}_Q * \bm{M}_K^T$ to calculate the attention maps, and the attention maps are combined with the labels. 

\subsubsection{\textbf{Saliency Token}}
\label{sec:3.2.8}
SnapMix~\cite{huang2020snapmix} used CAM to obtain feature maps of raw samples and mixed them with randomly generated masks. The ratio 
$\lambda$ was calculated based on the feature information in the mask region and the overall region ratio. Saliency Grafting ~\cite{park2021saliencygraft} extracted saliency maps using pre-trained CNNs, applied a softmax function, and used a threshold derived from the mean value of the saliency maps to generate a preliminary binary mask.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figs/SSL.pdf}
    \caption{\textbf{Left:} The framework of Vanilla CL and the CL with mixup. Vanilla CL used two different $\mathcal{A}(\cdot)$ for the same raw samples as ``positive'' samples, Mixup + CL used mixup and augmentation, aiming to obtain ``semi-positive'' samples. \textbf{Right:} The framework of Vanilla MAE and MAE with mixup. Vanilla MAE used an encoder and decoder to reconstruct the masked images into raw images. Mixup + MAE used mixed samples and decoded them into raw samples with an UnMix way.}
    \vspace{-10pt}
    \label{fig: ssl}
\end{figure}

\subsection{Self-Supervised Learning}
\label{sec:ssl}
\subsubsection{\textbf{Contrastive Learning}}
Contrastive learning (CL) has emerged as a prominent training paradigm in SSL, aiming to map similar ``positive" samples close to an ``anchor" and disparate ``negative" samples farther away. Mixup methods are widely used in CL to generate diverse or challenging samples. Fig. \ref{fig: ssl} illustrates the vanilla CL, vanilla MAE and two pipeline of them with mixup.

\textbf{Loss Object Improvement.}
MixCo~\cite{kim2020mixco} argued that mixed samples with semi-positive features help in learning better representations. Using CL with positive and negative samples and targets of mixed samples alleviates the instance discrimination problem by enabling the model to learn implicit relationships between positives and negatives (Eq. \ref{eq:22}).
\begin{equation}
    \label{eq:22}
    \begin{aligned}
    \mathcal{L}_{MixCo} & = - \sum_{i=1}^{N}(\lambda \cdot \log(\frac{\exp(\frac{\hat{z}_i \cdot z_i}{\tau})}{\textstyle \sum_{n=1}^{N}\exp(\frac{\hat{z}_i \cdot z_n}{\tau})})) + ((1-\lambda) \cdot \log(\frac{\exp(\frac{\hat{z}_i \cdot z_k}{\tau})}{\textstyle \sum_{n=1}^{N}\exp(\frac{\hat{z}_i \cdot z_n}{\tau})})),
    \end{aligned}
\end{equation}
where the $\tau$ denotes the softening temperature for similarity logits, $N$ is the number of mixed samples. 
Unlike MixCo, \emph{i}-Mix~\cite{lee2020i-mix} proposed inserting virtual labels for both the batch size and mixed samples at the input and label levels. It transforms unsupervised loss functions into supervised losses (\emph{e.g.}, CE losses) according to Eq. \ref{eq:23}:
\begin{equation}
    \label{eq:23}
    \begin{aligned}
    \mathcal{L}_{SimCLR} = - \log \frac{\exp(s(\hat{z}_i, z_{(N+i) \ \textrm{mod} \ 2N})/\tau)}{\textstyle \sum_{k=1, k\neq i}^{2N}\exp(s(\hat{z}_i , z_k)/\tau)},
    \ \
    \mathcal{L}_{N-pair} = - \sum_{n=1}^{N} \textrm{w}_{i,n} \log \frac{\exp(s(\hat{z}_i, z_n)/\tau)}{\textstyle \sum_{k=1}^{N}\exp(s(\hat{z}_i , z_k)/\tau)},
    \end{aligned}
\end{equation}
where $N$ is the batch size. Similar to \emph{i}-Mix, MCL ~\cite{wickstrom2022mcl} proposed a CL framework based on label smoothing principles. This framework employed a novel contrastive loss function to enhance the classification efficacy of clinical medicine time series data using a mixup to generate new samples.

SAMix~\cite{li2021samix} proposed improved infoNCE, $\mathcal{L}_{+}$ and $\mathcal{L}_{-}$, for mixup-based SSL. $\mathcal{L}_{+}$ is called the local term since features of another class are added to the original infoNCE loss; $\mathcal{L}_{-}$ is called the global term, and is the mixed infoNCE by Eq. \ref{eq:25}:
\begin{equation}
    \label{eq:25}
    \begin{aligned}
    \mathcal{L}_{+} & = - \lambda \log \hat{p}_{i} - (1 - \lambda) \log \hat{p}_{j}, \quad
    \hat{p}_{i} = \frac{\exp(\hat{z} \ z_i/\tau)}{\exp(\hat{z} \ z_i/\tau) + \exp(\hat{z} \ z_j/\tau)}.
    \end{aligned}
\end{equation}

Since SimSiam~\cite{chen2021simsiam} relies on pairs from the same sample's random augmentation, which can have high mutual information, it may reduce discriminative power for images with large intra-class variations, Guo \emph{et al.} proposed MixSiam~\cite{guo2021mixsiam} maximizes the significance of two augmented samples by inputting them into the encoder and aggregating the most significant representations. Another branch uses mixed samples as inputs, aiming for model predictions close to discriminative representations. This allows the model to access more varied samples and predict their most significant feature representations.

\textbf{Hard Sample Mining.}
In CL, training with hard samples can enhance model performance. MoCHi ~\cite{kalantidis2020mochi} improves performance by encoding raw samples to obtain representations, computing and ranking feature similarity with positive samples, and selecting the $N$ features with the lowest similarity for Manifold Mixup. This process generates more challenging negative samples.
Similarly, Co-Tuning~\cite{zhang2021co-tuneing}  proposed a contrastive regularization method to generate and mine hard sample pairs. BSIM~\cite{chu2020bsim} improved classification by measuring the joint similarity between raw and mixed samples (\emph{i.e.}, semi-positive pairs).  
FT~\cite{2020mocov2} introduced Positive Extrapolation \& Negative Interpolation to enhance MoCo~\cite{2020mocov2}. Positive Extrapolation uses Manifold Mixup to increase the difficulty of the \emph{Memory Bank}, while Negative Interpolation employs Mixup to generate mixed samples, increasing the diversity of negative samples.

In Graph CL, the most challenging negatives might be misclassified as false negatives if selected solely based on similarity to the anchor. ProGCL~\cite{xia2021progcl} stated that similarity alone cannot assess negative sample difficulty and proposed ProGCL-weight to prevent positive samples from being classified as challenging negatives. ProGCL-mix was then introduced to generate more true negatives. Unlike ProGCL, which is limited to graph tasks, DACL~\cite{verma2021dacl} proposed a domain-agnostic CL approach using noise samples to generate challenging sample pairs through mixed samples. The CL formulation uses a random sample $x_r$ to satisfy the condition $s(z_i, \hat{z}) > s(z_i, z_r)$, where $s(\cdot)$ is a cosine similarity function between two vectors.

\textbf{Application with Mixup and CL.} 
CoMix~\cite{sahoo2021comix} and MixSSL~\cite{zhang2022mixssl} used similar ideas for domain adaptation by mixing samples from different domains within the Contrastive Self-Supervised Learning framework for videos and medical images {m}-Mix~\cite{zhang2021m-mix} proposed mixing multiple samples and dynamically assigning different $\lambda$ to mine hard negative samples. Un-Mix~\cite{shen2022un-mix} noted that domain adaptation only changes the distance between samples while keeping labels constant during training. In contrast, mixup methods adjust both the sample and label spaces, with controllable changes that can capture more detailed features from unlabeled samples.

Based on some crop and cut ways. 
PCEA~\cite{liu2021pcea} proposed using four samples from different augmentation operations, pasting them together, and then cropping them into four individual samples, with two randomly selected for CL training. Similarly, Li \emph{et al.} proposed the Center-wise Local Image Mixture (CLIM)~\cite{li2020clim} method within a CL framework. After identifying cluster centers, CutMix is used to mix images from the same class and different resolutions, considering these as positive sample pairs.
CropMix~\cite{han2022cropmix} crops an image multiple times using different scales to capture multi-scale information and address the issue of information loss with single random crops. New input distributions are formed by blending multiple crop views, augmenting the input, and reducing label mismatches. The main encoder in CL can be based on both CNNs and ViTs.
PatchMix~\cite{shen2023patchmix} argued that existing contrastive frameworks overlook inter-instance similarities, such as different views of the same image. By leveraging ViTs, PatchMix randomly combines multiple images from a small batch at the patch level to generate mixed image patches, simulating rich inter-instance similarities in natural images. To improve ViT performance, SDMP~\cite{ren2022sdmp} treats mixed samples as additional positive pairs in SSL by modeling the semantic relationships and share the same source.

\subsubsection{\textbf{Masked Image Modeling}}
Masked Autoencoder (MAE)~\cite{he2022mae} uses Masked Image Modeling (MIM) to map tokens into a semantic space with an encoder and reconstruct original pixels with a decoder. MAE methods~\cite{li2022a2amim} showcase the powerful feature extraction and reconstruction capabilities of the encoder and decoder. $i$-MAE~\cite{zhang2022i-mae} investigates two main questions: (a) Are the latent space representations in masked autoencoders linearly separable? (b) To what extent do MAEs encode semantics in the latent feature space? $i$-MAE demonstrated that masked mixed samples can be reconstructed using two independent linear layers. However, reconstructing semantic similarity and achieving intra-class separation remains challenging, requiring knowledge of high-level visual concepts. Experiments show that MAEs are potent in the latent feature space.
MixMAE~\cite{liu2023mixmae}  combined the strengths of SimMIM~\cite{xie2022simmim} and MAE by encoding and decoding patch-level mixed samples. Instead of dropping all non-self-patches, it uses limited information during encoding and masks non-self-patches during decoding to prevent feature entanglement. A patch merging module is used to integrate feature information. Similarly, MixedAE~\cite{chen2023mixedae} increases the number of patches from two to four and introduces a Multi-head Homo Attention module, using the Homo Contrastive method for encoding and decoding. The Homo Attention module focuses on the highest-quality key patches using the top-$N$ approach. Homo Contrastive aims to enhance feature similarity of the same patches through supervised comparison.

\subsection{Semi-Supervised Learning}
\label{sec:semisl}
In deep learning tasks, it's easy to find numerous unlabeled samples $x_u$ but expensive to label them. Thus, researchers combine numerous unlabeled samples $x_u$ into a limited number of labeled samples $x$ for training the model to improve performance, called Semi-Supervised Learning (Semi-SL). Semi-SL avoids the waste of resources and solves the problems of poor generalization ability in SL and inaccuracy in SSL. Fig. \ref{fig: semisl_method} shows mixup methods' processes on Semi-SL tasks.

\textbf{Semi-SL.} MixMatch~\cite{berthelot2019mixmatch} is capable of guessing low-entropy labels for unlabeled examples and reduces the entropy of the labeling distribution $p$ by sharpening function: $p^{\frac{1}{\tau}}_i/ \sum_{i=1}^{L}p^{\frac{1}{\tau}}_i$, where temperature $\tau$ is a hyperparameter.
Pseudo labels were utilized to compute the unlabeled loss $\mathcal{L}_u$.
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.13]{Figs/SemiSL_method.pdf}
    \caption{Mixup methods used in SemiSL task. The top part is the pipeline of data labeling, and the bottom part is the model training using mixed samples.}
    \vspace{-10pt}
    \label{fig: semisl_method}
\end{wrapfigure}
ReMixMatch~\cite{kurakin2020remixmatch}  introduces two novel techniques, namely \textit{``Distribution Alignment''} and \textit{``Augmentation Anchoring''}, which are superimposed on top of the MixMatch. The objective of Distribution Alignment is to make the marginal distribution of predictions on unlabeled data closely match that of ground truth labels. Augmentation Anchoring involves introducing multiple strongly augmented input versions into the model, aiming to close each output to the prediction of a weakly augmented version of the same input. ICT~\cite{verma2022ict} calculated the consistency loss by comparing the prediction of mixed samples of unlabeled samples. 

Different from the previous method only considers predicted and pseudo-label. CowMask~\cite{french2020cowmask} used the teacher model to obtain pseudo-labels for raw samples and used CowMix to obtain predictions through the student model after obtaining mixed samples for consistency loss $\vert \hat{p}_s - p_t \vert{^2}$. The difference is that CowMask obtains the final pseudo-labels by performing a mix of pseudo-labels and the mean of the mask (as $\lambda$). $\epsilon$mu~\cite{pisztora2022emu} mixed labeled and unlabeled samples to obtain augmented samples, and instead of relating the labels of mixup directly to $\lambda$, the labels of mixup are instead adjusted using a hyperparameter $\lambda_{eps}$. The DCPA~\cite{chen2023dcpa} obtained a semi-supervised loss by predicting pseudo-labels using the teacher model, a supervised loss using mixed samples, and a contrasting loss using two different decoders that capture the variability of the features through a Sharpen operation, which is used to strengthen the consistency constraints, to bridge gaps in the outputs of the different decoders and to guide the learning direction of the model. MUM~\cite{kim2022mum} has developed a new approach to semi-supervised object detection that addresses the limitations of traditional data augmentation ways and aims to preserve the location information of the bounding box. MixPL~\cite{chen2023mixpl} proposed to compose the pseudo-labeled data by MixUp and Mosaic to soften the negative effect of missed detections and balance the learning at different scales.

\textbf{Label Noise Learning.} Unlike most existing Label Noise Learning (LNL) methods, DivideMix \cite{li2020dividemix} drops the labels of the samples that are most likely to be noisy and uses the noisy samples as unlabeled data to regularize the model, avoiding overfitting and improving the generalization performance. In addition, two networks are trained by co-divide at the same time. This keeps the two networks diverging so that different types of errors can be filtered and confirmation bias in self-training can be avoided. Manifold DivideMix~\cite{fooladgar2023mixematch} further improves DivideMix by selecting OOD samples and choosing noise samples based on the distribution of classification loss to find clean/noise samples to build a labeled/unlabeled dataset.

\textbf{Positive and Unlabeled Learning.} Positive and Unlabeled Learning (PUL) is a branch of Semi-SL that trains binary classifiers with only positive class and unlabeled data. Similarly, some mixup-based methods can improve the network's performance in PUL tasks. MixPUL~\cite{wei2020mixpul} combined supervised and unsupervised consistency training to create augmented samples. To promote supervised consistency, MixPUL further rewards unsupervised consistency between unlabeled samples by alleviating the supervised problem by mining reliable samples from the unlabeled set by identifying reliable negative sample subsets. In PUL tasks, the decision boundary often biases toward the positive class, resulting in some likely positive samples being mislabeled as negatives. This issue causes the decision boundary deviation phenomenon in PUL. P$^3$Mix~\cite{li2021yourp3mix} performs more accurate supervision by mixing unlabeled samples and positive samples from the decision boundary that are close to the boundary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  CV Downstream Tasks  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CV Downstream Tasks}
\label{sec:cvdownstream}
\subsubsection{\textbf{Regression}}
Regression tasks differ from classification ones as they need relatively accurate result prediction rather than class probability. So directly mixing two random samples may not make mixed samples effective for the model and can be harmful. MixRL ~\cite{hwang2021mixrl} proposed using the validation set to learn for each sample ``how many nearest neighbors to mix for best model performance''. Similar to AutoAugment~\cite{cubuk2018autoaugment}, Reinforcement Learning (RL) is used to find the lowest model loss on the validation set. Specifically, an RNN model determines the optimal number of KNNs for samples, and an MLP selects all the samples.

C-Mixup~\cite{yao2022c-mix} adjusts the sampling probability according to label similarity and selects sample pairs with similar labels for mixing. Vanilla MixUp's simple implementation leads to noisy samples and labels. For a selected sample, C-Mixup uses a symmetric Gaussian kernel to calculate another sample's sampling probability, with closer samples more likely to be sampled. Also, using low-dimensional label similarity for the calculation reduces the overhead.
Similarly to C-Mixup, ADA~\cite{schneider2024ada} uses a prior distribution for select samples and labels, UMAP Mixup~\cite{el2024umapmixup} uses the Uniform Manifold Approximation and Projection (UMAP) method as a regularizer to encourage and ensure that the mixup generates mixed samples that are on the flow of the feature and label data. ExtraMix~\cite{kwon2022extramix} proposed a mixup technique that can be extrapolated, expanding the latent space and label distribution. Compared to existing mixup-based methods, ExtraMix minimizes label imbalance. Warped Mix~\cite{bouniot2023warpedmixup} proposed a framework that takes similarity into effect when interpolating without dropping diversity. Warped Mix argued that similarity should influence the interpolation ratio $\lambda$, not the selection. High similarity should lead to a strong $\lambda$, and low similarity should lead to no change. SupReMix~\cite{wu2023supermix} aims to use better the inherent ``sequential" relationship between the inputs to facilitate the creation of ``harder" contrast pairs.

\subsubsection{\textbf{Long-tail Distribution}}
Data in nature often has long-tailed distributions. In deep learning, a superior model should handle this well. The augmented samples from mixup methods, with two different information features, seem to be well-suited for the long-tailed distribution problem.
Remix~\cite{chou2020remix} helps minority-class labels by giving them higher weights and allows feature and label differences in mixed samples for a better balance. UniMix~\cite{xu2021unimix} uses an improved mixed $\lambda$ and a sampler for minority classes, re-correcting fixed $\lambda$ with the UniMix factor based on prior-knowledge sampling for long-tail tasks.

OBMix~\cite{zhang2022obmix} uses two samplers $S_1$ and $S_2$ sampling independently to sample all the data classes in the dataset, generating a mini-batch with uniformly distributed classes, and then mixing to achieve the balance between the majority and minority classes. 
DBN-Mix~\cite{baik2024dbn-mix} combines two samples from the Uniform sampler and re-balance sampler modules to improve minority-class representation learning. Class-by-class Temperature scaling reduces classifier bias towards the majority class. As DBN-Mix generated samples are near minority-class boundaries (where data points are sparse), they better capture the minority-class distribution.

\subsubsection{\textbf{Segmentation}}
Image segmentation is a very crucial research and application in CV. Mixup methods are suitable for improving model performance in segmentation tasks as they preserve diverse samples. ClassMix~\cite{olsson2021classmix} used a pre-trained model as a teacher to obtain the masks of per labels and mixed different features obtained from the samples. To address some sites with a high level of symmetry, such as airports, ChessMix~\cite{pereira2021chessmix} proposed to mix the patches on samples in a chessboard-like grid to address the symmetry scenario. SA-MixNet~\cite{feng2024samix-net} pastes road areas from one image to another. Compared to other mixup methods, it retains road structural completeness. Additionally, a discriminator-based regularization method is designed to increase road connectivity while maintaining the structure. In Auto-Driving tasks, LaserMix~\cite{kong2023lasermix} and UniMix~\cite{zhao2024unimix} used the lidar dataset to mix samples.

Segmentation methods are widely used in medical images. CycleMix~\cite{zhang2022cyclemix} uses PuzzleMix to mix samples and randomly occlude patches. InsMix~\cite{lin2022insmix} applies morphological constraints to maintain clinical nuclear prior and utilizes background pixel redundancy. Smooth-GAN is proposed to harmonize the contextual information. DCPA~\cite{chen2023dcpa} and MiDSS~\cite{ma2024midss} use a pre-trained model to get pseudo labels for sample mixing. DCPA's student model has two decoders to capture feature variability after the Sharpen operation for contrasting loss, strengthening consistency, and guiding learning. ModelMix~\cite{zhang2024modelmix} constructs virtual models with convex combinations of convolutional parameters and regularizes the model set to minimize cross-task adjacency risk.

\subsubsection{\textbf{Object Detection}} 
MUM ~\cite{kim2022mum} (Mix \& UnMix) is proposed to improve semi-supervised teacher-student framework performance by mixing image blocks and reconstructing in feature space. Samples are sent to the teacher model for pseudo labels. Student model extracts features, mixes, and restores feature maps based on masks, generates predicted labels, and compares with pseudo labels for loss function. MixPL ~\cite{chen2023mixpl} uses the teacher model to generate pseudo-labels for both mixup and mosaic to get two different mixes of samples for training. Differing from obtained mixed samples, MS-DERT ~\cite{zhao2024msdert} proposed a new object detection architecture that mixed one-to-one and one-to-many supervision to improve the performance of models.


==> 4_Mixup_Methods4Other_tasks.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figs/other_applications.pdf}
    \caption{Illustration of other applications, we divided them into 9 detailed types.}
    \vspace{-10pt}
    \label{fig: other_app}
\end{figure*}
\section{Mixup for other applications}
\label{sec:mixup4other}
In this section, we discuss mixup-based methods applied to other tasks. As shown in Fig. \ref{fig: other_app}, we divided them into 2 main subsections: Traning Paradigms and Beyond Vision.

\subsection{Training Paradigms}
\subsubsection{\textbf{Federated Learning}}
Federated Learning (FL), initially proposed by Google in 2016, is a decentralized machine learning solution. It is designed to address data silos by training on distributed data in multiple endpoints to develop high-quality centralized models. To handle homo-distributed data, Shin \emph{at el.} propose XOR Mixup~\cite{shin2020xormixup}, which collects encoded data from other devices and decodes it using only each device's data, providing synthetic yet realistic samples for model training. The main idea is to use the property of dissimilarity operation: ($x_i$ $\oplus$ $x_j$) $\oplus$ $x_j$ = $x_i$, $x_i$ and $x_j$ from two individual devices. 

FedMix ~\cite{yoon2021fedmix} proposed the Mean Augmented Federated Learning (MAFL) framework, in which clients send and receive locally averaged data based on the privacy requirements of the target application to alleviate performance degradation caused by increased local data dissimilarity among clients.
Based on Federated Learning Distillation (FLD) and MixUp, Mix2FLD~\cite{oh2020mix2fld} is proposed. Specifically, each device uploads local model outputs like in FD and downloads model parameters like in FL to handle uplink-downlink channel asymmetry. Between the links, the server uses knowledge distillation to transfer the teacher's knowledge to the global model. However, the output-to-model conversion requires collecting additional training samples from the device, causing high communication overhead and violating local data privacy.
StatMix ~\cite{lewy2022statmix} computed image statistics ($\mu$ and $\sigma$ deviation of each color channel as content and style) for individual nodes, distributes the computed statistics to all nodes via a central server, and performs style delivery using these statistics in individual nodes.


\subsubsection{\textbf{Adversarial Attack \& Adversarial Training}}
Adversarial Attack \& Training ~\cite{szegedy2013adv} can significantly enhance model robustness by encouraging the model to explore unseen regions and OOD. Mixup methods also boost model performance and prevent overfitting. To improve model robustness, M-TLAT~\cite{laugros2020m-tlat} uses the MixUp in addition to a randomly generated dummy label, combines the mixed samples and their labels through a classifier to get the gradient perturbed noise $\delta$, and then mixes the noise and mixed samples to get the final augmented samples and labels according to the Eq. \ref{eq:28}:
\begin{equation}
    \label{eq:28}
    \begin{aligned}
    x_{adv} = \hat{x} - \epsilon * sign (\nabla_{\hat{x}} \mathcal{L}(\hat{x}, \hat{y}, \theta)),
    \end{aligned}
\end{equation}
where the $\epsilon * sign(\cdot)$ denotes the FGSM~\cite{iclr2015fgsm} or PGD~\cite{madry2017pgd} white box attack, and $\theta$ denotes the parameters of the models.

MI ~\cite{pang2019MI} converts the training stage to the inference stage by linearly mixing source samples with target samples noise-added by the adversarial attack. During the inference, it is optimal for MI compared to the direct use of an adversarial attack. Different from MI, AVMixup ~\cite{lee2020avmixup} adds perturbed noise at the input level and analyzes the effectiveness of soft-labeling on Adversarial Feature Overfitting (AFO). IAT ~\cite{lamb2019iat} combines clean sample loss and adversarial attack sample loss for training to get a better balance of robustness and accuracy. Similarly, Mixup-SSAT ~\cite{jiao2023mixup-ssat} explores the robustness of vehicle trajectory prediction and proposes a method that improves the model's robustness and decision-making ability for extreme cases by adding human-perturbed historical trajectories.
Not in image data modality, but in some text modality tasks, like text classification. Liu \emph{et al.} argued vanilla mixup's input-space linear restrictions often cause underfitting, especially with few training samples. Therefore, they proposed AMP ~\cite{liu2021amp}, adding an adversarial perturbation to the mixing ratio to relax the restrictions. AOM ~\cite{bunk2021aom} combines mixup methods and PGD adversarial optimization to get more robust classification models at the cost of a little accuracy. Si \emph{et al.} argued that in NLP tasks, the sample search space of simple adversarial training is hard to capture well. AMDA ~\cite{si2021amda} mixes in the latent space of the pre-trained model and uses the generated samples in the training stage to better cover the sample space and be closer to the raw sample distribution.

% \subsubsection{\textcolor{blue}{\textbf{Domain Adaption}}}
\subsubsection{\textbf{Domain Adaption}}
% Models trained on a specific domain typically demonstrate poorer performance when transferred to another domain. To address this issue, the domain adaptation strategy transfers model knowledge from the label-rich source domain to another label-scarce target domain. In the context of Unsupervised Domain Adaptation (UDA)~\cite{mao2019VMT,wu2020dmrl,yan2020iimt,xu2020dm-ada,sahoo2021comix,zhang2023samixup,zhang2022mixssl} and Partial Domain Adaptation (PDA)~\cite{sahoo2023slm}, there has been a notable push to enhance the effectiveness of models through the utilization of mixup ways for inter- or intra-domain data mixing.
Models trained on a specific domain often perform poorly when transferred to another domain. Domain adaptation strategies address this by transferring knowledge from a label-rich source domain to a label-scarce target domain. In the context of Unsupervised Domain Adaptation (UDA)~\cite{mao2019VMT,wu2020dmrl,yan2020iimt,xu2020dm-ada,sahoo2021comix,zhang2023samixup,zhang2022mixssl} and Partial Domain Adaptation (PDA)~\cite{sahoo2023slm}, there has been a significant effort to enhance model effectiveness using mixup methods for inter- or intra-domain data mixing.

% Virtual Mixup Training (VMT)~\cite{mao2019VMT}, as a regularization method, is capable of incorporating the locally-Lipschitz constraint into the region between the training data, rather than being constrained to the area around the training points by applying penalties to the difference between the prediction $p_i$ and the virtual label $y_i^v$.
Virtual Mixup Training (VMT)~\cite{mao2019VMT} is a regularization method that incorporates the locally-Lipschitz constraint between training data points, rather than just around the training points, by penalizing the difference between the prediction $p_i$ and the virtual label $y_i^v$.
Dual Mixup Regularization Learning (DMRL)~\cite{wu2020dmrl} to better ensure the discriminability of the latent space and extract domain-invariant features therein, the domain mixup regularization $\mathcal{L}^r_{adv}(\text{En}(x), \text{Dis}_d(x))$ and class mixup regularization $(\mathcal{L}^r_s(\text{En}(x), \text{Cls}(x))$ and $\mathcal{L}^r_t(\text{En}(x), \text{Cls}(x)))$ are incorporated into the traditional domain adversarial neural network according to Eq. \ref{eq:29}.
\begin{equation}
    \label{eq:29}
    \hspace{-0.5em}
    \begin{aligned}
        \mathop{\min}_{\text{En},\text{Cls}} \mathop{\max}_{\text{Dis}_d}
        \mathcal{L}(\text{En}(x), \text{Cls}(x)) + \textrm{w}_d\mathcal{L}_{adv}(\text{En}(x), \text{Dis}_d(x)), 
    \end{aligned}
\end{equation}
where $\text{En}(\cdot)$, $\text{Dis}_d(\cdot)$, and $\text{Cls}(\cdot)$ represent the feature extractor, domain discriminator, and classifier, respectively. $\mathcal{L}^r_{adv}(\text{En}(x), \text{Dis}_d(x))$ denotes the loss function that distinguishes features from the source or target domain, $\mathcal{L}^r_s(\text{En}(x), \text{Cls}(x))$ is used to assess the consistency loss between mixed source samples and their corresponding labels.

Domain Adaptation with Domain Mixup (DM-ADA)~\cite{xu2020dm-ada} ensures domain-invariance in the latent space, improving upon VAE-GAN~\cite{Larsen2015VAE_GAN} by constraining domain-invariance across source, target, and intermediate domains. Unlike DMRL~\cite{wu2020dmrl}, DM-ADA implements inter-domain data and latent space mixing and uses soft labels in the domain discriminator for evaluation.
IIMT~\cite{yan2020iimt} employs both intra-domain and inter-domain mixing within an adversarial learning framework to enforce training constraints. SLM~\cite{sahoo2023slm} eliminates negative migration by removing outlier source samples and learns discriminative invariant features through sample labeling and mixing, improving the PDA algorithm. CoMix~\cite{sahoo2021comix} proposed a CL framework for unsupervised video domain adaptation, using background mixing to create additional positives per anchor, thereby leveraging shared action semantics across domains.

In medical imaging, the Mixup Self-Supervised Learning (MixSSL)~\cite{zhang2022mixssl} framework enhances the robustness of classification models by mixing medical and natural image samples. SAMixup~\cite{zhang2023samixup} uses Domain-Distance-modulated Spectral Sensitivity (DoDiSS) to extract sensitive features across domains in the image phase.
Furthermore, it utilizes the DoDiSS map $z_s$ and adversarially learned parameter $\lambda_\theta$ as a weighting factor for cross-domain phase mixing operation:
\begin{equation}
    \label{eq:30}
    \begin{aligned}
        \hat{Am} = \lambda_\theta z_s Am^t + (1-\lambda_\theta) (1 - z_s) Am^s.
    \end{aligned}
\end{equation}

\subsubsection{\textbf{Knowledge Distillation}}
Knowledge Distillation (KD) uses a pre-trained teacher model to train a student model, offering an efficient paradigm for robust DNN training with less data and time. MixACM~\cite{muhammad2021mixacm} enhances this by passing mixed samples through both the teacher and student models to obtain intermediate features. These features are then mapped to activated channel maps, and the student model minimizes the inter-network loss to facilitate knowledge transfer.

MixSKD ~\cite{yang2022mixskd} integrates MixUp and Self-Knowledge Distillation into a unified framework. It uses the probability distribution from mixed images as a pseudo teacher distribution $f^\prime(\hat{x}_{i,j})$, guiding raw image pairs to produce consistent mixup predictions $\hat{p} = \lambda * f^\prime(x_i)+(1-\lambda) * f^\prime(x_j)$ in the network, achieving mutual distillation at both the feature and probability levels.
Moreover, MixKD ~\cite{choi2023mixkd} examines the impact of mixup augmentation on knowledge distillation and finds that ``smoothness'' is the key link. Experimental analysis suggests using a partial mixup (PMU) strategy in KD and scaling with the standard deviation as the temperature $\tau$.

\subsubsection{\textbf{LLM \& MLLM}}
Large Language Model (LLM) and Multi-modal Large Language Model (MLLM) has show its power ability based on numerous training data and huge parameters, has been successfully utilized in lots of tasks. 

\textbf{Basic multi-modal:} VLMixer~\cite{wang2022vlmixer} integrates Cross-modal CutMix (CMC) and contrastive learning to transform uni-modal text into multi-modal text  \& images, improving instance-level alignment between different modalities. CMC transfers natural sentences to multi-modality by randomly replacing vision-based words with semantically similar image patches, increasing data diversity while preserving semantic integrity. Oh \emph{at el.} found that despite CLIP's~\cite{radford2021clip} goal to align image and text embeddings, it maintains separate subspaces with large gaps, leading to poor uniformity and alignment even after fine-tuning, which limits embedding transferability and robustness. $m^2$-Mix ~\cite{oh2024m2-mix} addresses this by mixing image and text embeddings, generating hard-negative samples on the hyper-ball, and fine-tuning the model on hard-negative, raw, and positive samples using contrastive loss.
$\mathcal{P}$owMix~\cite{georgiou2023powmix} is an improvement of MultiMix, consists of five components: different number of mixing samples, mixing ratio reweighting, anisotropic/dynamic mixing, and cross-modal label mixing.

\textbf{LLMs/MLLMs:} MixGen ~\cite{hao2023mixgen} generates new image-text pairs by augmenting images with MixUp and linking texts to maintain semantic relationships. VQAMix~\cite{gong2022vqamix} proposes two approaches—ignoring mismatch mixed labels and conditional dynamic learning to adapt LLM to VQA data modality. This enables applying the Mixup method to VQA tasks. In LLM training, multi-domain corpora are commonly used. These corpora are often mixed based on human a priori knowledge. To identify an optimal mixing ratio, RegMix~\cite{liu2025regmix} trains small-scale proxy models based on small-scale corpora with different mixing ratios. Subsequently, a linear regression model is employed to predict the most suitable mixing ratio.
Beyond dataset-level mixing, researchers Zhou \emph{et. al.}\cite{zhou2025m3} proposed linearly interpolating the weight parameters of multiple LLMs, which were fine-tuned for different tasks. They posited the mixed LLM could inherit the capabilities of the original fine-tuned LLMs.

\subsection{Beyond Vision}
\subsubsection{\textbf{Natural Language Processing}}
NLP is a significant subfield of AI enabling computers to handle human language. Mixup methods are widely used in CV and explored in NLP to some extent, enhancing text data through mixing at sample, token, and hidden space levels.

\textbf{Text Classification.}
WordMixup \& SenMixup~\cite{guo2019WordMixup&SenMixu} propose two methods. WordMixup obtains mixed samples by linearly interpolating at the input level, while SenMixup mixes in the latent space (show in Fig. \ref{fig: NLP_method}). For different-length sentences, WordMixup padding sentences with zeros to the same length and interpolating the each dimensions of word. SeqMix~\cite{zhang2020seqmix} searches for matching sequences, mixes in feature and label, and uses a $\mathcal{D}(\cdot)$ to select sequences based on perplexity scores. Mixup-Transformer~\cite{sun2020mixup-transformer} passes sentences through a Transformer and linearly interpolates for classification. Seq-level Mix ~\cite{guo2020seq-level-mix} generates soft mixed samples by randomly combining sentence sub-parts, preventing memorization and encouraging reliance on sub-part composition for prediction.

MixText ~\cite{chen2020mixtext}, a semi-supervised method, generates augmented samples by mixing labeled and unlabeled text in the latent space. It minimizes the classification loss for labeled, unlabeled, and augmented samples, as well as the consistency loss between pseudo and ground truth labels. Similarly, EMix ~\cite{jindal2020EMix} uses interpolations of word embeddings and latent layer representations to construct virtual samples for sentence classification, reducing model overfitting. Notably, EMix uses the text standard deviation 
$\sigma$ to define the mixing ratio 
$\lambda_t$, accounting for text energy differences:
\begin{equation}
    \label{eq:31}
    \begin{aligned}
     &\hat{z} =\frac{\lambda_t z_i + (1- \lambda_t) z_j}{\sqrt{\lambda_t^2 + ( 1 - \lambda_t)^2}}, \ \lambda_t =\frac{1}{1+\frac{\sigma_i}{\sigma_j} \cdot \frac{1-\lambda}{\lambda}}.
    \end{aligned}
\end{equation}

Unlike previous methods, TreeMix ~\cite{zhang2022treemix} uses a constituency parsing tree to decompose sentences into sub-structures and recombine them to enhance sample diversity. However, assigning valid labels to augmented samples is challenging. TreeMix employs the proportion of words in new sentences as the mixup ratio for label convex combination:
\begin{equation}
    \label{eq:32}
    \begin{aligned}
     \hat{y}=\frac{L_i-|t^K_i|}{L_i-|t^K_i|+|t^L_j|}y_i+
     \frac{|t^L_j|}{L_i-|t^K_i|+|t^L_j|}y_j,
    \end{aligned}
\end{equation}
where $L$ is the length of sentence $x$ and $|t|$ is length of sub-sentences, $K$ is length of others. $L_i-|t^K_i|$ words from $x_i$ are kept and $|t^L_j|$ words from $x_j$ are inserted in new sentence.

Since the text consists of discrete tokens of variable length, applying MixUp to NLP tasks is an issue. Yoon \emph{et al.} proposed SSMix ~\cite{yoon2021ssmix}, optimized for NLP tasks by applying it at the input level instead of in the latent space. SSMix preserves the locality of raw texts by span-based mixing and uses saliency information to preserve more relevant tokens for prediction. $\max(\textrm{mix}(\lambda * x_i, x_j), 1)$ finds tokens of the same length for replacement. Different from WordMix, Nonlinear Mixup ~\cite{guo2020nonlinearmixup} uses a unique mixing $\lambda$ for each dimension of each word, changes samples and labels to nonlinear interpolation, and label mixing is based on input by adaptive learning. Specifically, for sentences $x \in \mathbb{R}^{\mathbb{N} \times C}$, and mixing with a matrix $\lambda \in \mathbb{R}^{\mathbb{N} \times C}$ element sampled independently.
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{-10pt}
    \includegraphics[scale=0.32]{Figs/NLP_method.pdf}
    \caption{Mixup methods used in text dataset for the text classification task. Two sentence embedding by Word2Vec~\cite{mikolov2013word2vec}, $x_i$, $x_j$ encoded and mixed their tokens.}
    \vspace{-10pt}
    \label{fig: NLP_method}
\end{wrapfigure}
\textbf{Neural Machine Translation.}
Neural Machine Translation (NMT) has significantly improved machine translation quality. Unlike traditional methods that generate diverse translations from a modeling perspective, MixDiversity~\cite{li2021MixDiversity} is a data-driven approach that enhances translation diversity by mixing different sentence pairs from the training set with source sentences during decoding. AdvAug~\cite{cheng2020advaug} proposes an adversarial augmentation method in NMT, replacing words to form adversarial samples and selecting them for convex combination over aligned word embeddings to enhance diversity and robustness. Multilingual Mix~\cite{cheng2022Multilingualmix} fuses two multilingual training examples using a multilingual crossover encoder-decoder to generate crossover examples that combine traits of different language pairs, improving cross-linguistic signal utilization. In cross-domain translation tasks, added noise in translated text is a common issue.
X-Mixup ~\cite{yang2022Xmixup} uses \emph{Scheduled Sampling} ~\cite{bengio2015scheduled} and \emph{Mixup Ratio} to handle the distribution shift and data noise problems respectively.

\textbf{Others.}
STEMM~\cite{fang2022stemm} processes speech and text samples using a w2t and a CNN to obtain semantic representations. Text samples are tokenized and passed through an embedding layer to get their representations. LADA~\cite{chen2020ladamixup}, similar to MixText, interpolates tokens in the hidden space for Named Entity Recognition. Pre-trained language models, due to their large number of parameters, may experience significant miscalibration between in-distribution and OOD data during fine-tuning. CLFT~\cite{kong2020clft} generates pseudo-on-manifold samples for in-distribution data calibration and pseudo-off-manifold samples for OOD data. Unlike other methods, HypMix~\cite{sawhney2021hypmix} proposes mixing in Riemannian hyperbolic space to avoid distortion and noise.

\subsubsection{\textbf{Graph Neural Network}}
Graph Convolutional Networks (GCN) have gained prominence due to their unique capabilities and are a major branch of deep learning. Traditional models excel with Euclidean data but struggle with non-Euclidean data. To address this, graphs represent non-Euclidean data, and GNNs process these graphs to extract features and patterns.
Xue \emph{et al.} proposed three augmentation methods~\cite{xue2021NodeAug-I} for GNNs: NodeAug-I, NodeAug-N, and NodeAug-S. NodeAug-I mixes the feature information and labels of two nodes to create new virtual nodes $v$ but ignores their edges. To address this, NodeAug-N and NodeAug-S were introduced. NodeAug-N creates virtual edges by selecting nodes with certain probabilities, while NodeAug-S generates new virtual edges by aggregating and scaling the directed edges of neighbors.
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[scale=0.20]{Figs/GraphMixup.pdf}
%     \caption{Mixup methods used for the graph classification task. The figure is reproduced from ~\cite{wu2021graphmixup}.}
%     \label{fig: GNN_method}
%     \vspace{-0.5em}
% \end{wrapfigure}
Unlike ~\cite{xue2021NodeAug-I}, MixGNN ~\cite{wang2021mixgnn} mixes receptive field subgraphs of randomly paired nodes and proposes a double-branch mixup GCN for interpolating irregular graph topologies. At each layer, GCN operates in two branches based on paired node topologies and aggregates the interpolated representations before the next layer. Both NodeAug-I and MixGNN mix at the input level, but they ignore the issue that sparse minority classes in graph samples may not be suitable for direct mixing.
PMRGNN ~\cite{ma2022PMRGNN} is a PageRank-based method for node classification tasks. It uses a PageRank-based random augmentation strategy, combines two encoders for cross-representation, and includes a graph regularization term. Graph Transplant ~\cite{park2022Graph-Transplant} proposes graph-level mixup by selecting nodes and edges with maximum saliency information and mixing them to create new edges, facilitating data-level mixing of irregular graphs.

Graphix~\cite{verma2021graphmix} uses GNNs to regularize the semi-supervised object classification, applies Manifold Mixup as data augmentation in the hidden layer, sharing parameters between the Fully-Connected Network and GNN to transfer discriminative node representations.
GraphSMOTE\cite{zhao2022GraphSMOTE} converts a sparse graph into a high-dimensional, dense representation using a GNN encoder. It selects a minority sample $x_i$ with embedding $z_i$, finds the nearest neighbor $z_n$ of the same label, and mixes the difference to create a new node $z_n$. A decoder predicts new edges $u$ for this node. GraphSMOTE uses the Synthetic Minority Over-sampling Technique (SMOTE) to create minority pseudo-examples and balance the training data.
Similarly, GraphMixup~\cite{wu2021graphmixup} proposes a semantic-level feature mixup with a reinforcement mechanism to address the class imbalance in node classification. iGraphMix ~\cite{jeong2023igraphmix} tackles irregularity and alignment issues in graph node classification by aggregating sampled neighbor nodes, demonstrating better generalization through theoretical analysis.

\subsubsection{\textbf{3D Point Cloud}}
PointMixup~\cite{chen2020pointmixup} addresses the problem that MixUp cannot be directly applied to point cloud tasks due to the lack of point correspondence. It defines point cloud data augmentation as the linear interpolation of shortest paths, using Earth Mover's 
Distance~\cite{rubner2000emd} to calculate shifts for matching points and create mixed samples by optimally assigning path functions between two data.

Some specific network architectures, \emph{e.g.}, PointNet++~\cite {qi2017pointnet++}, \emph{etc.}, focus on encoding local features, which results in PointMixup being prone to local ambiguity and non-natural results.
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.24]{Figs/PointCutMix.pdf}
    \caption{Visualization mixed samples based on 3D point clouds dataset, The figure reproduce from ~\cite{zhang2022pointcutmix}.}
    \vspace{-10pt}
    \label{fig: 3d_point}
\end{wrapfigure}
PointCutMix~\cite{zhang2022pointcutmix} addresses this by creating natural mixes by cutting and pasting subsets of two samples. RSMix~\cite{lee2021rs-mix} extends the 2D mask region concept to 3D, using KNN to maintain the point cloud shape and find similar neighbors, then extracts rigid subsets (RS) from each sample for mixing. Similar to RSMix and PointCutMix, PA-AUG~\cite{choi2021pa-aug} divides the data into 4 or 8 blocks and randomly applies five augmentation methods: dropout, CutMix, CutMix \& MixUp, sparse sampling, and random noise creation. Unlike hand-crafted methods, Point MixSwap ~\cite{umam2022point-mixswap} introduces a learnable Attention module that decomposes a point cloud into disjoint subsets, or divisions, and swaps corresponding divisions, resulting in highly diverse outputs.

\subsubsection{\textbf{Others}}
Since the mixup is a data-centric method, it can serve any model-centric task. 

\textbf{Signal Data Type:} Constrastive-mixup~\cite{zhang2022contrastive-mixup} uses mixup in speech recognition tasks, where two speech samples are mixed in the input-level and then classified, and unlike most mixup losses $\mathcal{L}_{MCE}$, Constrastive-mixup uses infoNCE loss for training. LLM~\cite{chang2023LLM} proposed a learnable loss function to obtain augmented samples by mixing samples with random noise. Octave Mix~\cite{hasegawa2021octave-mix} proposed to cross-process the low-frequency waveforms and high-frequency waveforms using frequency decomposition, extract the high and low-frequency information of $x_i$, $x_j$, respectively, cross-mix them, and then mix them by linear interpolation.

\textbf{Metric Learning:} 
To address the bias and extra overhead of hard negative samples in most CL methods, EE~\cite{ko2020ee} proposed learning loss metrics in the embedding space. It creates synthetic points with augmented information by combining feature points. Metrix~\cite{venkataramanan2021metrix} introduced a generalized formulation that encompasses existing metric learning loss functions.

\textbf{AI for Biological:} DNABERT-S~\cite{zhou2024dnabert-s} can efficiently cluster and separate different species in the embedding space. This improvement results from the proposed MI-Mix loss and Course Contrast Learning (C2LR) strategies. CL enables the model to distinguish between similar and dissimilar DNA sequences, and course learning progressively presents more challenging training samples, facilitating better learning and generalization.

\textbf{Low-level Task:}
Yoo \emph{et al.} found that spatial relationships are crucial in super-resolution tasks and proposed CutBlur~\cite{yoo2020cutblur}, which cuts Low-Resolution (LR) patches and pastes them into the corresponding High-Resolution (HR) regions. SV-Mixup~\cite{tan2023sv-mix} introduces a learnable selection module to choose the most informative volumes from two videos and mixes them to a new training videos for Video Action Recognition.
SiMix~\cite{patel2022simix} mixes two positive samples from the same mini-batch to form a virtual batch for training. In Unsupervised Continuous Learning (UCL) tasks, which often suffer from catastrophic forgetting, LUMP~\cite{madaan2021lump} improves model performance by selecting samples from buffer, mixing with the current sample. ContextMix~\cite{kim2024contextmix} combines mixup methods with static resized replacement to enhance performance.

==> 5_Analysis_and_Theorems.tex <==
\section{Analysis and Theorems}
\label{sec:analy&ther}
The mixup method has contributed to CV, NLP, \emph{etc.} Researchers are still exploring it. In this section, we summarize analyses and theorems about the mixup, focusing on (1). Hyperparameters and strategies in mixup (\emph{e.g.}, $\lambda$, mask, $\alpha$ selection). (2). Effects on model regularization (robustness, generalization). (3). Effects on improving model calibration exploration.

\subsection{Vicinal Risk Minimization}
\label{sec:vrm}
Supervised Learning aims to find a mapping function $f(\cdot)$ in a high-dimensional space that can model the relationship between an input random $x$ and an output random $y$ to a joint distribution $P(x,y)$ that is followed between $x$ and $y$. To keep the function $f$ constantly approximated, a loss function $\mathcal{L}$ is proposed to measure the difference between the model prediction $f(x)$ and the ground truth $y$. An optimization algorithm is also needed to minimize the average value of the loss function $\mathcal{L}$ over the joint distribution $P$ to obtain the optimal function $f^\star(\cdot)$:
\begin{equation}
\label{eq:33}
    \begin{aligned}
    f^\star = \textrm{argmin} \int \mathcal{L}(f(x), y)\textrm{d}P(x,y).
    \end{aligned}
\end{equation}

VRM~\cite{chapelle2000vrm} aims to fix the issues in Empirical Risk Minimization (ERM) that models tend to learn by the memory of the training data rather than generalizing it and have difficulty with OOD adversarial samples, turned the Eq. \ref{eq:34} into Eq. \ref{eq:35}:
\begin{equation}
\label{eq:34}
    \begin{aligned}
    \textrm{argmin} \int \mathcal{L}(f(x), y) \textrm{d}P_{\delta}(x,y)=\frac{1}{n} \sum_{i=1}^{n} \mathcal{L}(f(x_i, y_i)),
    \end{aligned}
\end{equation}
\begin{equation}
\label{eq:35}
    \begin{aligned}
    \textrm{argmin} \int \mathcal{L}(f(\hat{x}), \hat{y}) \textrm{d}P_{\mathcal{V}}(\hat{x},\hat{y})=\frac{1}{n} \sum_{i=1}^{n} \mathcal{L}(f(\hat{x}_i, \hat{y}_i)),
    \end{aligned}
\end{equation}
where the $P_{\delta}(x,y)= \frac{1}{n} \sum_{i=1}^{n} \delta(x = x_{i}, y = y_{i})$, and the $\delta(\cdot)$ denotes Dirac function. And for VRM, $P_{\mathcal{V}}(\hat{x},\hat{y}) = \frac{1}{n} \sum_{i=1}^{n} \mathcal{V}(\hat{x}, \hat{y} | x_i, y_i)$, $\mathcal{V}$ denotes the neighborhood distribution, used to measure the probability of the virtual sample pair ($\hat{x}, \hat{y}$) being found in the real sample pair ($x_i, y_i$).

\subsection{Hyperparameters \& Strategy}
In mixup methods, many hyperparameters can significantly impact the model's performance, \emph{e.g.} mixing ratio $\lambda$, mask $\mathcal{M}$, and $\alpha$ in Beta distribution. 

\textbf{Mixing Ratio \& Beta Distribution.}
Guo \emph{et al.} found that different mixing ratios impact model performance, leading to  \emph{``Manifold Intrusion"}. Experiments on the MINIST~\cite{lecun1998minist} dataset showed that a mixing ratio $\lambda$=0.5
resulted in worse performance compared to other ratios. AdaMixup~\cite{guo2018adamix} proposed using two individual models to create a mixing ratio $\lambda$ and identify mixed samples causing \emph{``Manifold Intrusion"}, aiming to reduce this issue. The mixing ratio $\lambda$ was sampled from a Beta($\alpha, \alpha$) distribution, with different hyperparameters $\alpha$ representing different curves. RegMixup~\cite{pinto2022regmixup} explored the relationship between $\alpha$ settings and model performance, proposing to combine CE loss and MCE loss to further improve performance, using MCE loss as a regularizer.

\textbf{Mask Policy \& Training Strategy.} 
Park \emph{et al.} proposed a unified theoretical analysis of mixed-sample data augmentation (MSDA), like MixUp and CutMix. Theoretical results show that input gradient and Hessians are regularized regardless of the mixing strategy. MSDA~\cite{park2022msda} combined MixUp and CutMix's advantages to design HMix and GMix. To solve the mixup's slow convergence and difficulty in selecting $\alpha$. Yu \emph{et al.} proposed the mixup Without hesitation (mWh) strategy~\cite{yu2021mwh}, which accelerates by periodically turning off the mix operation. Experimental analyses showed that mixup is effective in early epochs and not harmful in later ones. So, basic DA operations gradually replaced mixup, and model training shifted from exploration to utilization. Untied MixUp~\cite{archambault2019UntiedMixUp} claimed that mixup is similar to adversarial training. Adversarial training samples random noise and adds it to the source sample for training, enabling the model to learn features near the source sample distribution. Similarly, MixUp samples know ``noise'' and add it to the source sample for training. To perturb an instance $x_i$, DAT selects a random instance $x_j$, a random $\lambda$ from a given distribution, and perturbs $x_i$ to $x_j$ by a factor of (1 - $\lambda$) of the distance from $x_i$ to $x_j$.

\subsection{Robustness \& Generalization}
Mixup helps models learn robust features to prevent overfitting. By mixing samples, it makes models learn features for multiple classes simultaneously. Diverse samples improve generalization and performance on unseen data.

Liang \emph{et al.}~\cite{liang2018understanding} argued that there are two views to understanding mixup training. One of the views represented that mixup used linear interpolation of samples from different classes to create mixed samples. \textbf{Different linear interpolations created different samples, which gives the model more opportunities to sample features and avoid overfitting. This shows that the mixup is a DA method.} Another view represented that mixup allowed the model to learn multiple samples and avoid confusion between multiple samples so that \textbf{two different classes could be easily separated. This suggested that the mixup is a regularization.} 
For research on how mixup improves robustness and generalization,
Zhang \emph{et al.} provided theoretical analyses on how mixup improves robustness and generalization. For robustness, ~\cite{zhang2021howdose} demonstrated that the minimized mixup loss acts as a regularized version of standard empirical loss, leading to an upper bound on the two-step Taylor expansion to enhance adversarial robustness. For generalization, mixup serves as a data-adaptive regularization method, controlling Rademacher complexity~\cite{bartlett2001rademacher} to reduce overfitting. Similarly, ~\cite{carratino2022onmixupre} showed that mixup can be viewed as a standard EMR estimator, and that training with mixup is akin to learning from modified data with structured noise.

Liu \emph{et al.} reported a phenomenon in mixup training: on many general datasets, the performance of \textbf{mixup-trained models trained with numerous epochs begins to decay, creating a `U' curve}. This performance is further aggravated when the dataset samples are reduced. 
To understand mixup's performance, ~\cite{zhang2022when&how} theorized that mixup training adds labeling noise to mixed samples. Mixup improves generalization by initially fitting clean features but later overfits to noise, which can move model parameters away from the correct solution.
Teney \emph{et al.} found that selective mixup~\cite{teney2023selective-mix} is equivalent to resampling. They determined the limits of selective mixup, confirmed the effectiveness of resampling, and identified a better combination of their benefits.

\subsection{Model Calibration}
For some high-risk applications, the confidence of the Machine Learning model in its predictions is critical. Model calibration is to keep the predicted probability of the model results consistent with the true empirical probability. Where ECE~\cite{kuleshov2015ece} is one of the metrics. Manifold Mixup found that mixup can effectively improve the model calibration~\cite{guo2017calibration} metric as the ECE socre: $\mathrm{ECE}=\sum_{g=1}^{G} \frac{|B_g|}{n} |\operatorname{acc}(B_g)-\operatorname{conf}(B_g)|$,
where $n$ is the number of samples, the $B_g$ is the set of indices of samples whose prediction confidence falls into the interval $I_g$ = ( $\frac{g-1}{G}$,$\frac{g}{G}$], and $G$ denotes interval bins. The $\operatorname{acc}(B_g)$ and $\operatorname{conf}(B_g)$ as the Eq. \ref{eq:37}:
\begin{equation}
\label{eq:37}
    \begin{aligned}\hspace{-1.0em}
        \operatorname{acc}(B_g) = \frac{1}{|B_g|} \sum_{i \in B_g} (y_i, p_i), \
        \operatorname{conf}(B_g) = \frac{1}{|B_g|} \sum_{i \in B_g} p_i^c,
    \end{aligned}
\end{equation}
where the $y_i$ and $p_i$ denote the true class and predicted class, and $p_i^c$ is the confidence for sample $x_i$.


Thulasidasan \emph{et al.}~\cite{thulasidasan2019onmixup} argued that overconfidence or underconfidence in models arises from one-hot labels. Experiments with small-scale and large-scale image samples, as well as NLP samples, showed that using mixup results in label smoothing. This provides benefits beyond high accuracy, leading to better-calibrated models and reduced overconfidence, offering advantages over other label-smoothing methods.
Zhang \emph{et al.} demonstrated theoretically that mixup improves calibration in high-dimensional settings by investigating natural statistical models. The calibration benefits of mixup increase with model scale, supported by experiments on mainstream architectures and datasets. Mixup enhances calibration, especially when the number of parameters exceeds the number of samples. Additionally, ~\cite{zhang2022when&how} explored mixup's impact on calibration in Semi-SL. While mixing unlabeled samples led to poor calibration, adding mixup training alleviated this issue. Experiments showed that pseudo-labeling impairs calibration, but combining mixup with pseudo-labeling can improve it.


==> 6_Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This section bases our discussion on the following two points for mixup methods: challenge problems \& future works.

\subsection{Challenge Problems}
\label{sec: challenge problems}
Mixup mainly focuses on image classification tasks based on SL. Then it expands to other training paradigms (\emph{e.g.}, SSL, Semi-SL, FL, KD, MM, \emph{etc.}), and not only image classification but also on text, speech, graph, 3d point clouds tasks. Mixup has shown excellent robustness and generalization in all of these tasks, as well as improving model performance. However, there are still some problems with the current method that deserve to be explored and resolved in specific tasks and scenarios.
\begin{itemize}
    \item \textbf{Mixed Sample Generation \& Selection.}
    While generating reliable mixed samples has been extensively explored in discriminative tasks like classification, adapting these methods for LLMs demands fundamental redesign. Traditional methods rely on linear interpolation in fixed label spaces (\emph{e.g.}, MixUp, CutMix), whereas LLMs need to maintain the logic in context when using mixed samples. \textbf{Extending mixup to effectively generate or select reliable samples for models remains a key research challenge.}

    \item \textbf{Mixed Labels Improvement.} The mixing ratio $\lambda$ is pivotal in defining label semantics and loss computation in the mixup framework. At the sample level, learnable methods make the mask follow $\lambda$, at the label level, the mask recalculates $\lambda$. However, no metric exists to evaluate the correctness and reliability of these processes. \textbf{Meanwhile, improving mixup label quality could be crucial to a general, high-performance, efficient method than modifying sample generation.} 

    \item \textbf{Trade-off between Performance \& Efficiency.} AutoMix has achieved a good trade-off for vision tasks, but the problem persists. This is the case not only for mixups but also for some general DA methods. Some offline methods can reduce the overhead but are not generalizable to other scenarios, in contrast, some online methods can adaptively generalize to other scenarios but also increase the overhead of model training. \textbf{The optimal data augmentation is to obtain more gains in less time and generalize to more tasks.}

    \item \textbf{Alleviating Mainfold Intrusion \& OOD Detection.} Since mixup involves features of two or more classes, it easily causes ``Manifold Intrusion'', which destroys the data manifold in high-dimensional space during mixing, making the model less robust and unreliable. For OOD, some mixup methods use extra images as ``noise'' to enhance OOD detection ability, but this is input-level-based and limited by design. \textbf{How to reduce ``Manifold Intrusion'' and design a more adaptive OOD detection method, especially within the framework of LLMs, is worth further exploration.}

    \item \textbf{Transfer to Unified mixup Framework.} Although there are lots of mixup methods in different tasks and scenarios, those mainly proposed for specific tasks are hard to transfer to others. Mainstream mixup methods are proposed for image classification, and with some downstream task transfer experiments in object detection or segmentation. However, these are based on image modality and are not effective for others, \emph{e.g.}, text, speech, and protein. Thus, \textbf{how to transfer mixup methods to a unified framework is an issue worth being explored and studied.}

\end{itemize}

\subsection{Future Works}
\label{sec: future works}
As an augmentation method, mixup can be applied in lots of tasks. What specific tasks can be performed as part of a \emph{``data-centric''} method, taking into account the latest technologies and discoveries, and we outline some opportunities.
\begin{itemize}
    \item \textbf{Number of samples to Mix.} Most mixup methods use 2 sample mixes. In image classification, Co-Mix\cite{kim2020co}, AdAutoMix\cite{qin2023adautomix} instead chooses mixing 2-3 samples for improving model performance. However, for other tasks, there is no option to mix multiple samples. Mixing multiple samples can further increase the diversity of the augmented samples and, at the same time, lead to the sample difficulty. Thus, it is worthwhile research to find and choose the number of mixed samples for the corresponding task.

    \item \textbf{Applying on MLLMs and Mixup.} MLLMs have shown a powerful capability. $m^2$-Mix used the text \& image modality mixing to improve CLIP\cite{radford2021clip}. Different data modalities with various features could bring more features and reduce the gap between different modalities, which can enhance the robustness and generalization of the model when trained with image, text, and audio mixed samples.

    \item \textbf{Generating samples based on Generative Model.} GAN\cite{goodfellow2020gans}, VAE\cite{kingma2013vae}, Diffusion Model (DM)\cite{ho2020ddpm} can generate high-quality samples and some current work such as DiffuseMix\cite{islam2024diffusemix}, DiffMix\cite{wang2024diffmix} have demonstrated that generative models can be used as a DA method. However, DM needs a lot of time to generate samples. GAN and VAE can generate them quickly, but the quality of the generated samples is difficult to ensure. How to trade the efficiency and quality is worthwhile to research.

    \item \textbf{Employing a Unified Mixup Framework.} Mixup as a plug-and-play, simple, and effective DA tool initially. It has now become a trainable \& end-to-end way. We argue that mixup is not considered a tool anymore, but a training framework. However, most researchers still as the bias that mixup as the DA method, designing it according to the tasks they need to perform. We call for applying mixups as a unified framework to achieve more tasks specifically.

\end{itemize}

==> 7_Conclusion.tex <==
\section{Discussion}
\label{sec:conclusion}
In this survey, we reformulate mixup methods as a unified framework and summarise those methods' technical details and data modalities on various tasks from 2018 to 2025. In addition, we divided mixup into two main classes: Sample Mixup Policies and Label Mixup Policies, which could contain different improved versions of mixup, and conclude all mixup methods in this survey as two Figures: Fig. \ref{mixup4cv} and Fig. \ref{mixup4other}. Also, we summarize the various types of datasets frequently used in mixup methods, the classification results of some mainstream mixup methods for image classification tasks in SL on commonly used datasets based on mainstream models that are displayed in Table \ref{tab:CNN-based_results}, Table \ref{tab:ViT-based_results} and Table \ref{Dataset}. Finally, we discuss existing problems and worthwhile future works to give researchers some advanced ideas and thoughts in this field.


% \section*{Acknowledgement}
% This work was supported by National Key R\&D Program of China (No. 2022ZD0115100), National Natural Science Foundation of China Project (No. U21A20427), and Project (No. WU2022A009) from the Center of Synthetic Biology and Integrated Bioengineering of Westlake University. This work was done by Xin Jin, Hongyu Zhu, and Zedong Wang during their internship at Westlake University.



==> Tabs/datasets_wo_cite.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{0.5mm}
    \caption{Summary of frequently used datasets for mixup methods tasks. \href{https://github.com/Westlake-AI/Awesome-Mixup}{Link} to dataset websites is provided.}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l c c c c c } \hline
    Dataset  & Type & Label & Task & Total data number & Link \\ \hline
    MINIST & Image & 10 & Classification & 70,000 & \href{https://yann.lecun.com/exdb/mnist/}{MINIST} \\
    Fashion-MNIST & Image & 10 & Classification & 70,000 & \href{https://github.com/zalandoresearch/fashion-mnist}{Fashion-MINIST} \\
    CIFAR10 & Image & 10 & Classification & 60,000 & \href{https://www.cs.toronto.edu/~kriz/cifar.html}{CIFAR10} \\
    CIFAR100 & Image & 100 & Classification & 60,000 & \href{https://www.cs.toronto.edu/~kriz/cifar.html}{CIFAR100} \\
    SVHN & Image & 10 & Classification & 630,420 & \href{http://ufldl.stanford.edu/housenumbers/}{SVHN} \\
    GTSRB & Image & 43 & Classification & 51,839 & \href{https://benchmark.ini.rub.de/gtsrb_dataset.html}{GTSRB} \\
    STL10 & Image & 10 & Classification & 113,000 & \href{https://cs.stanford.edu/~acoates/stl10/}{STL10} \\
    Tiny-ImageNet & Image & 200 & Classification & 100,000 & \href{http://cs231n.stanford.edu/tiny-imagenet-200.zip}{Tiny-ImageNet} \\
    ImageNet-1K & Image & 1,000 & Classification & 1,431,167 & \href{https://image-net.org/challenges/LSVRC/2012/}{ImageNet-1K} \\
    CUB-200-2011 & Image & 200 & Classification, Object Detection & 11,788 & \href{https://www.vision.caltech.edu/datasets/cub_200_2011/}{CUB-200-2011} \\
    FGVC-Aircraft & Image & 102 & Classification & 10,200 & \href{https://www.robots.ox.ac.uk/~vgg/data/fgvc-aircraft/}{FGVC-Aircraft} \\
    StanfordCars & Image & 196 & Classification & 16,185 & \href{https://ai.stanford.edu/$/sim20jkrause/cars/car_dataset.html}{StanfordCars} \\
    Oxford Flowers  & Image & 102 & Classification & 8,189 & \href{https://www.robots.ox.ac.uk/~vgg/data/flowers/102/}{Oxford Flowers} \\
    Caltech101  & Image & 101 & Classification & 9,000 & \href{https://data.caltech.edu/records/mzrjq-6wc02}{Caltech101} \\
    SOP  & Image & 22,634 & Classification & 120,053 & \href{https://cvgl.stanford.edu/projects/lifted_struct/}{SOP} \\
    Food-101  & Image & 101 & Classification & 101,000 & \href{https://data.vision.ee.ethz.ch/cvl/datasets_extra/food-101/}{Food-101} \\
    SUN397  & Image & 899 & Classification & 130,519 & \href{https://vision.princeton.edu/projects/2010/SUN//}{SUN397} \\
    iNaturalist  & Image & 5,089 & Classification & 675,170 & \href{https://github.com/visipedia/inat_comp/tree/master/2017}{iNaturalist} \\
    CIFAR-C  & Image & 10,100 & Corruption Classification & 60,000 & \href{https://github.com/hendrycks/robustness/}{CIFAR-C} \\
    CIFAR-LT  & Image & 10,100 & Long-tail Classification & 60,000 & \href{https://github.com/hendrycks/robustness/}{CIFAR-LT} \\
    ImageNet-1K-C  & Image & 1,000 & Corruption Classification & 1,431,167 & \href{https://github.com/hendrycks/robustness/}{ImageNet-1K-C} \\
    ImageNet-A  & Image & 200 & Classification & 7,500 & \href{https://github.com/hendrycks/natural-adv-examples}{ImageNet-A} \\
    Pascal VOC 102  & Image & 20 &  Object Detection & 33,043 & \href{http://host.robots.ox.ac.uk/pascal/VOC/}{Pascal VOC 102} \\
    MS-COCO Detection  & Image & 91 & Object Detection & 164,062 & \href{https://cocodataset.org/detection-eval}{MS-COCO Detection} \\
    DSprites  & Image & 737,280$\times$6 & Disentanglement & 737,280 & \href{https://github.com/google-deepmind/dsprites-dataset}{DSprites} \\
    Place205  & Image & 205 & Recognition & 2,500,000 & \href{http://places.csail.mit.edu/downloadData.html}{Place205} \\
    Pascal Context  & Image & 459 & Segmentation & 10,103 & \href{http://places.csail.mit.edu/downloadData.html}{Pascal Context} \\
    ADE20K  & Image & 3,169 & Segmentation & 25,210 & \href{https://groups.csail.mit.edu/vision/datasets/ADE20K/}{ADE20K} \\
    Cityscapes  & Image & 19 & Segmentation & 5,000 & \href{https://deepmind.google/}{Cityscapes} \\
    StreetHazards  & Image & 12 & Segmentation & 7,656 & \href{https://www.v7labs.com/open-datasets/streethazards-dataset}{StreetHazards} \\
    PACS  & Image & 7$\times$4 & Domain Classification & 9,991 & \href{https://domaingeneralization.github.io/}{PACS} \\
    \hline
    
    BRACS  & Medical Image & 7 & Classification & 4,539 & \href{https://www.bracs.icar.cnr.it/}{BRACS} \\
    BACH  & Medical Image & 4 & Classification & 400 & \href{https://iciar2018-challenge.grand-challenge.org/}{BACH} \\
    CAME-Lyon16  & Medical Image & 2 & Anomaly Detection & 360 & \href{https://camelyon16.grand-challenge.org/}{CAME-Lyon16} \\
    Chest X-Ray  & Medical Image & 2 & Anomaly Detection & 5,856 & \href{https://data.mendeley.com/datasets/rscbjbr9sj/2}{Chest X-Ray} \\
    BCCD  & Medical Image & 4,888 & Object Detection & 364 & \href{https://github.com/Shenggan/BCCD_Dataset}{BCCD} \\
    TJU600  & Palm-Vein Image & 600 & Classification & 12,000 & \href{https://cslinzhang.github.io/ContactlessPalm/}{TJU600} \\
    VERA220  & Palm-Vein Image & 220 & Classification & 2,200 & \href{https://www.idiap.ch/en/scientific-research/data/vera-palmvein}{VERA220} \\
    \hline

    CoNLL2003  & Text & 4 & Classification & 2,302 & \href{https://data.deepai.org/conll2003.zip}{CoNLL2003}\\
    20 Newsgroups  & Text & 20 & OOD Detection & 20,000 & \href{http://qwone.com/~jason/20Newsgroups/}{20 Newsgroups} \\
    WOS  & Text & 134 & OOD Detection & 46,985 &\href{http://archive.ics.uci.edu/index.php}{WOS} \\
    SST-2  & Text & 2 & Sentiment Understanding & 68,800 &\href{https://github.com/YJiangcm/SST-2-sentiment-analysis}{SST-2} \\
    \hline

    Cora  & Graph & 7 & Node Classification & 2,708 & \href{https://github.com/phanein/deepwalk}{Cora}\\
    Citeseer  & Graph & 6 & Node Classification & 3,312 & \href{https://csxstatic.ist.psu.edu/}{CiteSeer}\\
    PubMed  & Graph & 3 & Node Classification & 19,717 & \href{https://pubmed.ncbi.nlm.nih.gov}{PubMed}\\ 
    BlogCatalog & Graph & 39 & Node Classification & 10,312 & \href{https://figshare.com/articles/dataset/BlogCatalog_dataset/11923611?file=22349970}{BlogCatalog}\\ 
    \hline
    
    Google Commands  & Speech & 30 & Classification & 65,000 & \href{https://research.google/blog/launching-the-speech-commands-dataset/}{Google Commands} \\
    VoxCeleb2  & Speech & 6,112 & Sound Classification & 1,000,000+ & \href{https://www.robots.ox.ac.uk/~vgg/data/voxceleb/}{VoxCeleb2} \\
    VCTK  & Speech & 110 & Enhancement & 44,000 & \href{https://datashare.ed.ac.uk/handle/10283/2791}{VCTK} \\
    \hline
    
    ModelNet40  & 3D Point Cloud & 40 & Classification & 12,311 & \href{https://modelnet.cs.princeton.edu/}{ModelNet40} \\
    ScanObjectNN  & 3D Point Cloud & 15 & Classification & 15,000 & \href{https://hkust-vgd.github.io/scanobjectnn/}{ScanObjectNN} \\
    ShapeNet  & 3D Point Cloud & 16 & Recognition, Classification & 16,880 & \href{https://shapenet.org/}{ShapeNet} \\
    KITTI360  & 3D Point Cloud & 80,256 & Detection, Segmentation & 14,999 & \href{https://www.cvlibs.net/datasets/kitti/}{KITTI360} \\
    \hline

    UCF101  & Video & 101 & Action Recognition & 13,320 & \href{https://www.crcv.ucf.edu/research/data-sets/ucf101/}{UCF101} \\
    Kinetics400  & Video & 400 & Action Recognition & 260,000 & \href{https://deepmind.google/}{Kinetics400} \\
    \hline
    
    Airfoil  & Tabular & - & Regression & 1,503 & \href{https://archive.ics.uci.edu/dataset/291/airfoil+self+noise}{Airfoil} \\
    NO2  & Tabular & - & Regression & 500 & \href{https://drive.google.com/drive/folders/1pTRT7fA-hq6p1F7ZX5oJ0tg_I1RRG6OW}{NO2} \\
    Exchange-Rate  & Timeseries & - & Regression & 7,409 & \href{https://github.com/laiguokun/multivariate-time-series-data}{Exchange-Rate} \\
    Electricity  & Timeseries & - & Regression & 26,113 & \href{https://github.com/laiguokun/multivariate-time-series-data}{Electricity} \\
    \hline
    \end{tabular}
    }
    \label{Dataset}
\end{table}

==> arXiv/mixup4cv.tex <==
\tikzstyle{my-box}=[
 rectangle,
 draw=hidden-draw,
 rounded corners,
 text opacity=1,
 minimum height=1.5em,
 minimum width=5em,
 inner sep=2pt,
 align=center,
 fill opacity=0.5,
 ]
 \tikzstyle{leaf}=[my-box, minimum height=1.5em,
 fill=hidden-blue!60, text=black, align=left,font=\scriptsize,
 inner xsep=2pt,
 inner ysep=4pt,
 ]
\begin{figure*}[t]
	\centering
	\resizebox{\textwidth}{!}{
		\begin{forest}
			forked edges,
			for tree={
    				grow=east,
    				reversed=true,
    				anchor=base west,
    				parent anchor=east,
    				child anchor=west,
                        node options={align=center},
                        align=center,
    				base=left,
    				font=\small,
    				rectangle,
    				draw=hidden-draw,
    				rounded corners,
    				% minimum width=4em,
    				edge+={darkgray, line width=1pt},
    				s sep=3pt, 
    				inner xsep=2pt,
    				inner ysep=3pt,
    				ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
			},
			where level=1{text width=5.6em,font=\scriptsize}{},
			where level=2{text width=5.5em,font=\scriptsize}{},
			where level=3{text width=4.0em,font=\scriptsize}{},
            where level=4{text width=6.3em,font=\scriptsize}{}, 
			[
			Mixup Methods for CV tasks, ver
			[
			Supervised \\ Learning
    			[
    			Sample Mixup \\ Policies
                        [
                        Ad-Hoc
                            [
                            Static Linear
                                [
                			    MixUp{\cite{zhang2018mixup},}
                                BC{\cite{cvpr2018bc},}
                                LocalMixup{\cite{baena2022localmixup},}
                                AugMix{\cite{hendrycks2019augmix},}
                                PixMix{\cite{hendrycks2022pixmix},}
                                DJMix{\cite{hataya2020djmix},}
                                IPMix{\cite{huang2024ipmix}}
                                , leaf, text width=31em
                                ]
                            ]
                            [
                            Feature-basd
                                [
                    		Manifold Mixup{\cite{verma2019manifold},}
                    		PatchUp{\cite{faramarzi2020patchup},}
                                MoEx{\cite{li2021moex},} 
                                Catch-up Mix{\cite{kang2024catchupmix}}
                                , leaf, text width=31em
                                ]
                            ]
                            [
                            Cutting-basd
                                [
                    		CutMix{\cite{yun2019cutmix},}
                                MixedExamples{\cite{summers2019mixedexamples}}
                    		Pani Mixup{\cite{sun2024panimixup},} 
                                FMix{\cite{harris2020fmix},} 
                                GridMix{\cite{Baek2021gridmix},}
                                SmoothMix{\cite{lee2020smoothmix},} \\
                                ResizeMix{\cite{qin2020resizemix},} 
                                StackMix{\cite{chen2022stackmix},}
                                SuperpixelGridMix{\cite{hammoudi2022superpixelgridcut},}
                                MSDA{\cite{park2022msda},}
                                YOCO{\cite{han2022yoco},}
                                StarMix{\cite{jin2024starlknet}}
                                , leaf, text width=31em, align = left
                                ]
                            ]
                            [
                            K Samples \\ Mixup
                                [
                                Mosaic{\cite{redmon2016yolo},}
                                RICAP{\cite{takahashi2019ricap},} 
                    		$k$-Mixup{\cite{greenewald2021kmixup},}
                    		DCutMix{\cite{jeong2021dcutmix},}
                                MixMo{\cite{rame2021mixmo},}
                                Cut-thumbnail{\cite{xie2021Cut-thumbnail}}
                                , leaf, text width=31em
                                ]
                            ]
                            [
                            Random Policies
                                [
                    		RandomMix{\cite{liu2024randomix},}
                    		AugRMixAT{\cite{liu2022augrmixat}} 
                                , leaf, text width=31em
                                ]
                            ]
                        ]
                        [
                        Adaptive
                            [
                            Style-based
                                [ 
                                StyleMix{\cite{cvpr2021stylemix},} 
                                MixStyle{\cite{zhou2021mixstyle},}
                                AlignMixup{\cite{2021alignmix},}
                			    MultiMix{\cite{venkataramanan2022multimix}}
                                , leaf, text width=31em
                                ]
                            ]
                            [
                            Saliency-based
                                [
                    		SaliencyMix{\cite{uddin2020saliencymix},}
                    		Attentive-CutMix{\cite{icassp2020attentive},}
                                AttributeMix{\cite{li2020attributemix},}
                                PuzzleMix{\cite{kim2020puzzle},}
                                SuperMix{\cite{dabouei2021supermix},}
                                Co-Mix{\cite{kim2020co},} \\
                                SnapMix{\cite{huang2020snapmix},}
                                FocusMix{\cite{kim2020focusmix},}
                                AutoMix{\cite{liu2022automix},}
                                SAMix{\cite{li2021samix},}
                                RecursiveMix{\cite{yang2022recursivemix},} 
                                TransformMix{\cite{cheung2024transformmix},} \\
                                GraSalMix{\cite{hong2023gradsalmix},} 
                                GuidedMixup{\cite{kang2023guidedmixup},}
                                LGCOAMix{\cite{dornaika2023lgcoamix},}
                                AdAutoMix{\cite{qin2023adautomix}} 
                                , leaf, text width=31em, align=left
                                ]
                            ]
                            [
                            Attention-based
                                [
                			    TokenMixup{\cite{choi2022tokenmixup},}
                                TokenMix{\cite{liu2022tokenmix},}
                                ScoreMix{\cite{stegmuller2023scorenet},}
                			    MixPro{\cite{zhao2023mixpro},} 
                                SMMix{\cite{chen2023smmix}} 
                                , leaf, text width=31em
                                ]
                            ]
                            [
                            Generating \\ Samples
                                [
                                AAE{\cite{liu2018aae},}
                    		AMR{\cite{beckham2019amr},}
                                ACAI{\cite{berthelot2018acai},}
                    		AutoMixup{\cite{zhu2020automixup},}
                                VarMixup{\cite{mangla2020varmixup},}
                                DiffuseMix{\cite{islam2024diffusemix}} 
                                , leaf, text width=31em
                                ]
                            ]
                        ]
			      ]
    			[
    			Label Mixup \\ Policies
                        [
                        Ad-Hoc
                            [
                            Optimizing \\ Calibration
                                [
                                CAMixup{\cite{wen2020camix},}
                                RankMixup{\cite{noh2023rankmixup},} 
                                SmoothMixup{\cite{jeong2021smoothmixup}}
                                , leaf, text width=31em, align = left
                                ]
                            ]
                            [
                            Area-based
                                [
                                TransMix{\cite{chen2022transmix},}
                                RICAP{\cite{takahashi2019ricap},} 
                                RecursiveMix{\cite{yang2022recursivemix}}
                                , leaf, text width=31em, align = left
                                ]
                            ]
                            [
                            Loss Object
                                [
                                DecoupledMix{\cite{liu2022decoupledmix},}
                                MixupE{\cite{zou2023mixupe}} 
                                , leaf, text width=31em, align = left
                                ]
                            ]
                            [
                            Random Policies
                                [
                                mWH{\cite{yu2021mwh},}
                                RegMixup{\cite{pinto2022regmixup}}
                                , leaf, text width=31em, align = left
                                ]
                            ]
                        ]
                        [
                        Adaptive
                            [
                            Optimizing \\ Mixing ratio
                                [
                                AdaMixup{\cite{guo2018adamix},}
                                MetaMixup{\cite{mai2021metamixup},}
                                LUMix{\cite{sun2022lumix},}
                                SUMix{\cite{qin2024sumix}}
                                , leaf, text width=31em, align = left
                                ]
                            ]
                            [
                            Generating Label
                                [
                                GenLabel{\cite{sohn2022genlabel}}
                                , leaf, text width=31em,
                                ]
                            ]
                            [
                            Attention Score
                                [
                                Token Labeling{\cite{jiang2021tokenlabeling},}
                                TokenMixup{\cite{choi2022tokenmixup},}
                                TokenMix{\cite{liu2022tokenmix},}
                    		  Mixpro{\cite{zhao2023mixpro},} 
                                TL-Align{\cite{xiao2023tl-align}} 
                                , leaf, text width=31em, align=left
                                ]
                            ]
                            [
                            Saliency Token
                                [
                                Saliency Grafting{\cite{park2021saliencygraft},}
                                SnapMix{\cite{huang2020snapmix}}
                                , leaf, text width=31em, align=left
                                ]
                            ]
                        ]
    			]
			]
			[
			  Self-Supervised \\ Learning
    			[
    			  Contrastive \\ Learning
        			[
                        MixCo{\cite{kim2020mixco},}
                        MoCHi{\cite{kalantidis2020mochi},}
                        BSIM{\cite{chu2020bsim},}
                        \emph{i}-Mix{\cite{lee2020i-mix},}
                        MixSSL{\cite{zhang2022mixssl},}
                        FT{\cite{zhu2021ft},}
                        Co-Tuning{\cite{zhang2021co-tuneing},} 
                        CLIM{\cite{li2020clim},}
                        PCEA{\cite{liu2021pcea},} 
                        SAMix{\cite{li2021samix},} 
                        CoMix{\cite{sahoo2021comix},} \\
                        MixSiam{\cite{guo2021mixsiam},} 
                        Un-Mix{\cite{shen2022un-mix},}
                        \emph{m}-Mix{\cite{zhang2021m-mix},}
                        SDMP{\cite{ren2022sdmp},}
                        CropMix{\cite{han2022cropmix},}
                        MCL{\cite{wickstrom2022mcl},} 
                        ProGCL{\cite{xia2021progcl},}
                        PatchMix{\cite{shen2023patchmix},}
                        DACL{\cite{verma2021dacl},}
                        \emph{m$^2$}-Mix{\cite{oh2024m2-mix}}
                        , leaf, text width=44.6em, align=left,
        			]
    			]
                    [
    			Masked \\ Image Modeling
        			[
        			\emph{i-MAE}{\cite{zhang2022i-mae},}
                        MixMAE{\cite{liu2023mixmae},}
                        MixedAE{\cite{chen2023mixedae}}
        			, leaf, text width=44.6em
        			]
                    ]
			]
			[
			Semi-Supervised \\ Learning
    			[
    			  SemiSL
        			[
            		MixMatch{\cite{berthelot2019mixmatch},}
                        ReMixMatch{\cite{kurakin2020remixmatch},}
                        DivideMix{\cite{li2020dividemix},}
                        MixPUL{\cite{wei2020mixpul},}
                        CowMask{\cite{french2020cowmask},}
                        $\epsilon$mu{\cite{pisztora2022emu},}
                        P$^3$Mix{\cite{li2021yourp3mix},}
                        ICT{\cite{verma2022ict},}
                        DCPA{\cite{chen2023dcpa},}
                        MixPL{\cite{chen2023mixpl},} \\
                        Manifold DivideMix{\cite{fooladgar2023mixematch},}
                        MUM{\cite{kim2022mum},}
                        DecoupledMix{\cite{liu2022decoupledmix},}
                        LaserMix{\cite{kong2023lasermix}}
        			, leaf, text width=44.6em, align=left
        			]
    			]	
			]
			[
			  Downstream \\ Tasks
    			[
                    Regression
                        [
                        MixRL{\cite{hwang2021mixrl},}
                        C-Mixup{\cite{yao2022c-mix},}
                        ADA{\cite{schneider2024ada},}
                        ExtraMix{\cite{kwon2022extramix},}
                        SupReMix{\cite{wu2023supermix},}
                        Warped Mixup{\cite{bouniot2023warpedmixup},}
                        UMAP Mixup{\cite{el2024umapmixup}}
                        , leaf, text width=44.6em
                        ]
    			]
                    [
                    Long-tail \\ Distribution
                        [
                        Remix{\cite{chou2020remix},}
                        UniMix{\cite{xu2021unimix},}
                        OBMix{\cite{zhang2022obmix},}
                        DBN-Mix{\cite{baik2024dbn-mix}}
                        , leaf, text width=44.6em
                        ]
    			]
                    [
                    Segmentation
                        [
                        ClassMix{\cite{olsson2021classmix},}
                        ChessMix{\cite{pereira2021chessmix},}
                        CycleMix{\cite{zhang2022cyclemix},}
                        InsMix{\cite{lin2022insmix},}
                        LaserMix{\cite{kong2023lasermix},}
                        DCPA{\cite{chen2023dcpa},}
                        SA-MixNet{\cite{feng2024samix-net},}
                        MiDSS{\cite{ma2024midss},} 
                        UniMix{\cite{zhao2024unimix},} \\
                        ModelMix{\cite{zhang2024modelmix}}
                        , leaf, text width=44.6em, align=left
                        ]
    			]
                    [
                    Object Detection
                        [
                        MUM{\cite{kim2022mum},}
                        MixPL{\cite{chen2023mixpl},}
                        MS-DERT{\cite{zhao2024msdert}}
                        , leaf, text width=44.6em
                        ]
    			]
			]
		      ]
		\end{forest}
  }
\caption{Summary of mixup methods for CV tasks, including SL, SSL, Semi-SL, and some downstream tasks (Regression, Long-tail, Segmentation, and Object Detection).}
\label{mixup4cv}
\end{figure*}


==> arXiv/mixup4other.tex <==
\tikzstyle{my-box2}=[
 rectangle,
 draw=hidden-draw-green,
 rounded corners,
 text opacity=1,
 minimum height=1.5em,
 minimum width=5em,
 inner sep=2pt,
 align=center,
 fill opacity=0.5,
 ]
 \tikzstyle{leaf}=[my-box2, minimum height=1.5em,
 fill=hidden-green!60, text=black, align=left,font=\scriptsize,
 inner xsep=2pt,
 inner ysep=4pt,
 ]
\begin{figure*}[t]
	\centering
	\resizebox{\textwidth}{!}{
		\begin{forest}
			forked edges,
			for tree={
    				grow=east,
    				reversed=true,
    				anchor=base west,
    				parent anchor=east,
    				child anchor=west,
                        node options={align=center},
                        align=center,
    				base=left,
    				font=\small,
    				rectangle,
    				draw=hidden-draw-green,
    				rounded corners,
    				% minimum width=4em,
    				edge+={darkgray, line width=1pt},
    				s sep=3pt, 
    				inner xsep=2pt,
    				inner ysep=3pt,
    				ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
			},
			where level=1{text width=5.6em,font=\scriptsize}{},
			where level=2{text width=5.5em,font=\scriptsize}{},
			% where level=3{text width=4.0em,font=\scriptsize}{},
            % where level=4{text width=6.0em,font=\scriptsize}{}, 
			[
			Mixup Methods for other applications, ver
            [
            Training \\ Paradigms
                [
                Federated \\ Learning
                    [
                    XOR Mixup{\cite{shin2020xormixup},}
                    FedMix{\cite{yoon2021fedmix},}
                    Mix2Fld{\cite{oh2020mix2fld},}
                    StatMix{\cite{lewy2022statmix}}
                    , leaf, text width=44.3em, align=left,
                    ]
                ]
                [
                Adversarial \\ Attack/Training
                    [
                    M-TLAT{\cite{laugros2020m-tlat},}
                    MI{\cite{pang2019MI},}
                    AVMixup{\cite{lee2020avmixup},}
                    AMP{\cite{liu2021amp},}
                    AOM{\cite{bunk2021aom},}
                    AMDA{\cite{si2021amda},}
                    IAT{\cite{lamb2019iat},}
                    Mixup-SSAT{\cite{jiao2023mixup-ssat}}
                    , leaf, text width=44.3em, align=left,
                    ]
                ]
                [
                Domain \\ Adaption
                    [
                    MixSSL{\cite{zhang2022mixssl},}
                    CoMix{\cite{sahoo2021comix},}
                    VMT{\cite{mao2019VMT},}
                    IIMT{\cite{yan2020iimt},}
                    DM-ADA{\cite{xu2020dm-ada},}
                    DMRL{\cite{wu2020dmrl},}
                    SLM{\cite{sahoo2023slm},}
                    SAMixup{\cite{zhang2023samixup}}
                    , leaf, text width=44.3em, align=left,
                    ]
                ]
                [
                Knowledge \\ Distillation
                    [
                    MixACM{\cite{muhammad2021mixacm},}
                    MixSKD{\cite{yang2022mixskd},}
                    MixKD{\cite{choi2023mixkd}}
                    , leaf, text width=44.3em, align=left,
                    ]
                ]
                [
                Multi-Modal
                    [
                    VLMixer{\cite{wang2022vlmixer},}
                    MixGen{\cite{hao2023mixgen},}
                    \emph{m$^2$}-Mix{\cite{oh2024m2-mix},}
                    $\mathcal{P}$owMix{\cite{georgiou2023powmix},}
                    DiffMix{\cite{wang2024diffmix}}
                    , leaf, text width=44.3em, align=left,
                    ]
                ]
            ]
            [
            Beyond \\ Vision
                [
        		NLP
            		[
            		WordMixup \& SenMixup{\cite{guo2019WordMixup&SenMixu},}
                    SeqMix{\cite{zhang2020seqmix},}
                    Mixup-Transformer{\cite{sun2020mixup-transformer},}
                    CLFT{\cite{kong2020clft},}
                    EMix{\cite{jindal2020EMix},}
                    MixText{\cite{chen2020mixtext},}
                    Seq-Level Mix{\cite{guo2020seq-level-mix},}
                    AdvAug{\cite{cheng2020advaug},} \\
                    Nonlinear Mixup{\cite{guo2020nonlinearmixup},}
                    LADA{\cite{chen2020ladamixup},} 
                    MixDiversity{\cite{li2021MixDiversity},}
                    SSMix{\cite{yoon2021ssmix},}
                    HypMix{\cite{sawhney2021hypmix},}
                    STEMM{\cite{fang2022stemm},}
                    TreeMix{\cite{zhang2022treemix},}
                    AdMix{\cite{jin2022admix},} 
                    X-Mixup{\cite{yang2022Xmixup},} \\
                    Multilingual Mix{\cite{cheng2022Multilingualmix}}
                    , leaf, text width=44.3em, align=left,
            		]
        		]
        		[
        		GNN
                    [
            	NodeAug-I{\cite{xue2021NodeAug-I},}
                    MixGNN{\cite{wang2021mixgnn},}
                    PMRGNN{\cite{ma2022PMRGNN},}
                    GraphSMOTE{\cite{zhao2022GraphSMOTE},}
                    GraphMix{\cite{verma2021graphmix},}
                    GraphMixup{\cite{wu2021graphmixup},}
                    Graph Transplant{\cite{park2022Graph-Transplant},}
                    G-Mixup{\cite{han2022g-mix},} \\
                    iGraphMix{\cite{jeong2023igraphmix}}
                    , leaf, text width=44.3em, align=left,
            		]
        		]
        		[
        		3D Point
            		[
                    PointMixup{\cite{chen2020pointmixup},}
                    PointCutMix{\cite{zhang2022pointcutmix},}
                    RS-Mix{\cite{lee2021rs-mix},}
                    PA-AUG{\cite{choi2021pa-aug},}
                    Point MixSwap{\cite{umam2022point-mixswap}}
                	, leaf, text width=44.3em, align=left
            		]	
        		]
                [
        		Others
            		[
                    SiMix{\cite{patel2022simix},}
                    Constrastive-mixup{\cite{zhang2022contrastive-mixup},}
                    LLM{\cite{chang2023LLM},}
                    EE{\cite{ko2020ee},}
                    Metrix{\cite{venkataramanan2021metrix},}
                    LUMP{\cite{madaan2021lump},}
                    Octave Mix{\cite{hasegawa2021octave-mix},}
                    CutBlur{\cite{yoo2020cutblur},} 
                    SV-Mixup{\cite{tan2023sv-mix},} \\
                    DNABERT-S{\cite{zhou2024dnabert-s},}
                    ContextMix{\cite{kim2024contextmix},}
                    OpenMixup{\cite{2022openmixup}}
                	, leaf, text width=44.3em, align=left
            		]	
        		]
            ]
		    ]
		\end{forest}
  }
\caption{Summary of mixup methods for other applications, including training paradigms and beyond vision (Text, Graph, 3D Point, Audio, \emph{ect}).}
\label{mixup4other}
\end{figure*}


==> pkgs.tex <==
% IEEE default packages
\usepackage{tikz}
\usepackage{amsmath}
\usepackage{filecontents}
%\usepackage{calc}
\usepackage[flushleft]{threeparttable}
%\usepackage{cite}
\usepackage{float}
\usepackage{amsmath,amsfonts}
% argmax and argmin
\DeclareMathOperator*{\argmin}{\arg\min}
\DeclareMathOperator*{\argmax}{\arg\max}
% \usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
% \newcommand{\V}{\checkmark}
% pkg loaded already in USENIX
% \usepackage[usenames,dvipsnames]{xcolor}

% for bib citations
%\usepackage[numbers,sort&compress]{natbib}
\usepackage{url}
\def\UrlBreaks{\do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J
\do\K\do\L\do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V
\do\W\do\X\do\Y\do\Z\do\[\do\\\do\]\do\^\do\_\do\`\do\a\do\b
\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n
\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z
\do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]\do\)\do\,
\do\?\do\'\do+\do\=\do\#} 

\usepackage{lipsum,tabularx}
\usepackage{wrapfig}
% \usepackage{breakurl}
\usepackage{multicol}
\usepackage{multirow}
% \usepackage{amssymb}

% for good looking tables
\usepackage{colortbl}
\usepackage{booktabs}
\usepackage{setspace}

% for autoref and settings
% pkg hyperref loaded in USENIX
% \usepackage[hidelinks,breaklinks,colorlinks]{hyperref}
% \hypersetup{
%     linkcolor={blue!70!black},
%     citecolor={red!70!black},
%     urlcolor={blue!70!black}
% }
\def\Snospace~{\S{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}
\renewcommand{\figurename}{Fig.}
\def\figureautorefname{\figurename}
\newcommand{\subfigureautorefname}{\figureautorefname}
\newcommand{\algorithmautorefname}{Algorithm}

% font encoding using T1
\usepackage[T1]{fontenc}
\usepackage{pifont}
% for math macro and numbers
% \usepackage{fp}
% \usepackage{siunitx}
% \usepackage{amsmath,amsopn,amssymb}
\newcommand*\TC[1]{%
  \begin{tikzpicture}[baseline=(C.base)]
    \node[draw,circle,inner sep=0.2pt](C) {\textcolor{black}{#1}};
  \end{tikzpicture}
}
% pseudo code

% \usepackage{minted}
% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage[noend]{algpseudocode}
% balance bibliography
\usepackage{balance}

% math
\usepackage{bm}
\usepackage{fp}
\usepackage{siunitx}
% use \num{123456} -> 123,456
\sisetup{group-separator={,},group-minimum-digits={3},output-decimal-marker={.}}

% definition
\usepackage{amsthm}
% \newtheorem{definition}{Problem}
% \newtheorem{definition}{Definition}

% for captions and subfigures
% \usepackage[labelfont=bf,font=small,skip=5pt]{caption}
\usepackage[labelfont=bf,font=small,skip=5pt]{caption}
% \usepackage{subcaption}
% \renewcommand\thesubfigure{(\alph{subfigure})}
% \captionsetup[sub]{labelformat=simple}

% for commenting a large section
\usepackage{comment}

% lastpage for page N of M
% \usepackage{lastpage}

% fancy header
\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\cfoot{\thepage}

%% others
% \usepackage{endnotes,microtype,xspace,graphicx,fancyvrb,multirow}
% \usepackage{array,underscore,relsize}
% \usepackage{enumitem}

%%
%% NOTE.
%%  to use circled number in caption, use
%%   (e.g., \protect\WC{1})
%%
\usepackage{tikz}
\newcommand*\WC[1]{%
  \begin{tikzpicture}[baseline=(C.base)]
    \node[draw,circle,inner sep=0.2pt](C) {#1};
  \end{tikzpicture}
}

\newcommand*\BC[1]{%
  \begin{tikzpicture}[baseline=(C.base)]
    \node[draw,circle,fill=black,inner sep=0.2pt](C) {\textcolor{white}{#1}};
  \end{tikzpicture}
}

% % Spacing
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\abovedisplayshortskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}
% \setlength{\jot}{0pt}

% sema
\usepackage{xspace}
\newcommand{\shl}{\ \cc{<}\cc{<}\ }
\newcommand{\shr}{\ \cc{>}\cc{>}\ }
\newcommand{\x}{$\times$\xspace}
\newcommand{\V}{\checkmark}
\newcommand{\X}{{\footnotesize $\times$}\xspace}
\renewcommand{\O}{\phantom{0}}

% boxbeg/end
\newcommand{\boxbeg}{
  \vspace{2px}
  \noindent\begin{tabular}{|l|}\hline
    \begin{minipage}{3.2in}
      \vspace{2px}
      \noindent
      }

      \newcommand{\boxend}{
      \vspace{2px}
    \end{minipage} \\ \hline
  \end{tabular}
  \vspace{-10pt}
}
\usepackage{listings}
% algorithm in paper
% \usepackage{algorithm}
% \usepackage[ruled]{algorithm2e}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% cite line
% \usepackage{algpseudocode}
% \usepackage[algcompatible]{algpseudocode}

% \newcommand{\coo}{\ensuremath{\mathrm{CO_2}}}

\usepackage[edges]{forest}
\usepackage{cancel}
% \usepackage{microtype}

\definecolor{hidden-draw-green}{RGB}{92,226,194}
\definecolor{hidden-draw}{RGB}{106,142,189} 
\definecolor{hidden-blue}{RGB}{194,232,247} 
\definecolor{hidden-green}{RGB}{202,246,229}

\usepackage[normalem]{ulem}
\useunder{\uline}{\ul}{}
